A Continuous Time GARCH(p,q) Process with Delay

We investigate the properties of a continuous time GARCH process as the solution to a L\'evy driven stochastic functional integral equation. This process occurs as a weak limit of a sequence of discrete time GARCH processes as the time between observations converges to zero and the number of lags grows to infinity. The resulting limit generalizes the COGARCH process and can be interpreted as a COGARCH process with higher orders of lags. We give conditions for the existence, uniqueness and regularity of the solution to the integral equation, and derive a more conventional representation of the process in terms of a stochastic delayed differential equation. Path properties of the volatility process, including piecewise differentiability and positivity, are studied, as well as second order properties of the process, such as uniform L1 and L2 bounds, mean stationarity and asymptotic covariance stationarity.

==> WIP/WIP.tex <==
%!TEX root = ../WIP.tex
\tableofcontents
\newpage\section{Coding}
\begin{enumerate}
	\item Inputs:
	\begin{enumerate}
		\item Time parameters:
		\begin{enumerate}
			\item Discretization: $\delta\in(0,1)$
			\item Horizon: $T>0$
			\item Delays: $p,q\ge 0$
		\end{enumerate}
		\item Noise sequence: $(L_n, S_n)_{n\in\{-r/\delta, \ldots ,T/\delta\}}$ from $( b_L, \sigma^2_L, \Pi_L)$ and $(\delta, T, p, q)$
		
		\item Process parameters
		\begin{enumerate}
			\item CDGARCH $\eta, c_\mu, c_\nu$
			\item Discretized $f_\mu$ and $f_\nu$ in the form $f(-k \delta)$
		\end{enumerate}
		
		
	\end{enumerate}
	\item Outputs:
	\begin{enumerate}
		\item Processes: $X_n$, $Y_n$
		\item Moments?
	\end{enumerate}

	\item Programs:

	
	
	 
\end{enumerate}

\begin{enumerate}
	\item \verb|main.m|
	\begin{enumerate}
		\item Specify parameters:
			\begin{enumerate}
				\item Time: $\delta, T, p,q$
				\item CDGARCH: $\eta, c_\mu, c_\nu, \norm{f_\mu}_1, \norm{f_\nu}_1, \Pi_L$
			\end{enumerate}
		\item \verb|par_time|
			=\verb|par_time.m| $(\delta, p, q, T)$ 

		Compute the grid and positions of points
		
		\item \verb|par_CDGARCH| = \verb|CDGARCH.m|($\delta$, \verb|par_time|, $\eta, c_\mu, c_\nu, \norm{f_\mu}_1, \norm{f_\nu}_1,  \Pi_L$)

		Assume $f$ is constant, then $f_\mu(u) = \ind_{[-p,0]}(u) \norm{f_\mu}_{1}/p$, want $p/\delta$ points.

		\item $(\Delta X,\Delta Y)=\verb|CDGARCH.m|(\delta, grid, f_\delta, noise)$
		\begin{enumerate}
			\item Noise: $\verb|par_noise|$
		\end{enumerate}

		\item $(\Delta L,\Delta S)=\verb|noise.m|(\delta, \verb|grid|, \verb|par_noise|)$ 
		
			
	\end{enumerate}
\end{enumerate}



	

% %%%%%%%%%%%%%%%%%%%%DIFFERENT VERSION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{lemma}\label{lemma/1/stationarity/cross}
% 	Suppose Assumptions \ref{assumptions/1/existence} hold and $(X_t)_{t\ge 0}$ is the unique strong solution to \eqref{equation/1/stationarity/X} with initial condition $\Phi$. 
% 	Let $k\ge 1$, then
% 	\begin{align*}
% 		\Em\left[X_t^{k-1}\int_{t-r}^t f(u-t)X_u du \right]
% 		\le \norm{f_\mu}_{1}\left( \frac{k-1}{k} \Em[X_t^k]
% 		+\frac{1}{k} \sup_{u\in[t-r,t]}\Em[X_u ^k]\right).
% 	\end{align*}
% 	Suppose further $S\in \cH^k\loc$, i.e., $\kappa_{2k}<\infty$. Then for all $t>0$,
% 	there exists a constant $C_k = C_{k,S,f,t}$ such that
% 	\begin{align*}
% 		\Em \left[X_t^{k-1} \int_{t-q+}^t f_\nu(u-t) X_{u-} d\td S_u\right]
% 		\le \frac{k-1}{k}\Em[X_t^k]
% 		+\frac{C_k}{k} \norm{f_\nu}_{k}^k \sup_{u\in(t-q,t]}\Em[X_u ^k].
% 	\end{align*}
% 	In the case where $k=1,2$,  we can choose $C_1=0$ and $C_2 = \kappa_4$.

% 	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 	\begin{proof}
% 	Recall Young's inequality $xy\le \frac{1}{p}x^{p} + \frac{1}{q} y^{q}$,  for all  $x,y,p,q>0$  with $\frac{1}{p}+\frac{1}{q}=1$. By   Fubini's Theorem and Young's inequality,
% 	\begin{align*}
% 		&\Em \left[X_t^{k-1} \int_{t-r}^t f(u-t) X_u  du\right]
% 		=\int_{t-r}^t f(u-t) \Em \left[X_t^{k-1} X_u \right] du
% 		   \\
% 		& \hspace{1cm}		\numberthis\label{equation/1/proofs/1/stationarity/pqUI/bound_on_du_integral}
% 		\le \norm{f_\mu}_{1}\sup_{u\in[t-r,t]} \Em \left[ X_t^{k-1}  X_u \right]
% 		\le \norm{f_\mu}_{1}\left( \frac{k-1}{k} \Em[X_t^k]
% 		+\frac{1}{k} \sup_{u\le t}\Em[X_u ^k]\right).
% 	\end{align*}
% 	For the second claim, Young's inequality and Theorem 66 on page 346 of \cite{Protter2004} gives
% 	\begin{align*}
% 		&\Em \left[X_t^{k-1} \int_{t-q+}^t f_\nu(u-t) X_{u-} d\td S_u\right]
% 		\le \Em \left[\frac{k-1}{k} X_t^k 
% 		+ \frac{1}{k}\left(\int_{t-q+}^t f_\nu(u-t) X_{u-} d\td S_u\right)^k \right]
% 		\\
% 		&\hspace{3cm} \le\frac{k-1}{k}\Em[X_t^k]
% 		+\frac{C_k}{k}  \int_{t-q+}^t f_\nu(u-t)^k \Em[X_u ^k] du
% 		   \\
% 		& \hspace{3cm} \le\frac{k-1}{k}\Em[X_t^k]
% 		+\frac{C_k}{k} \norm{f_\nu}_{k}^k \sup_{u\in(t-q,t]}\Em[X_u ^k],
% 	\end{align*}
% 	for some $C_k$ which depends on $S, f$ and $t$. For the case $k=2$, simply observe that
% 	\begin{align*}
% 		\Em\left[\left(\int_{t-q+}^t f_\nu(u-t) X_{u-} d\td S_u\right)^2 \right]
% 		= \kappa_4  \int_{t-q}^t f_\nu(u-t)^2 \Em\left[X_u ^2\right] du
% 	\end{align*}
% 	so we could choose $C_2= \kappa_4$. The $k=1$ case is trivial. 
% 	\end{proof}
% \end{lemma}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{proof}[Proof of Theorem \ref{theorem/1/stationarity/moment bound} (\ref{theorem/1/stationarity/Lk pq})]
% Fix $k\ge 1$, by Ito's Lemma applied to $x\mapsto x^{k}$, 
% 	\begin{align*}
% 		dX_t^{k} = k X_t^{k-1} dX_t
% 		+ \frac{k(k-1)}{2}X_t^{k-2 }d[X,X]_t,
% 	\end{align*}
% 	where from \eqref{equation/1/stationarity/p0X},  $d[X,X]_t = c_\nu^2 X_{t-} d[\td S, \td S]_t$. 
% 	Writing $E(t) := \Em\left[X_t^{k}\right]$, we have
% 	\begin{align*}
% 		E(t)  =E(0)
% 		+& k \Em\left[\int_0^t X_s^{k-1} 
% 		\Big(\eta - c_0 X_s + \Xi(X)_s\Big)ds \right]
% 		+\frac{k(k-1)}{2}
% 		\kappa_4 c_\nu ^2 \Em\left[\int_{0}^t X_s^{k } ds\right],
% 	\end{align*}
% 	which after rearranging becomes
% 	\begin{align*}
% 		E(t)&= E(0) 
% 		+k\Em\left[ \int_0^t X_s^{k-1}
% 		 \left( \eta+ \left( \frac{k-1}{2} \kappa_4 c_\nu ^2 - c_0\right) X_s \right) ds\right]
% 		   \\
% 		& \qquad  
% 		+ k\Em\left[ \int_0^t X_s^{k-1} \left(\int_{s-p}^s f(u-s)X_u  du +\int_{s-q+}^s f(u-s)X_{u-} d\td S_u\right) ds 
% 			\right].
% 		\numberthis\label{equation/1/proofs/1/stationarity/pqUI/E(t)}
% 	\end{align*}
% 	For the first integral in \eqref{equation/1/proofs/1/stationarity/pqUI/E(t)}, recall our assumed condition
% 	\begin{align*}
% 		\lambda:= \frac{1}{2}\left(c_0 - \frac{k-1}{2} \kappa_4 c_\nu^2 
% 						- \frac{k-1}{k} - \norm{f_\mu}_{1} - \frac{C_k}{k} \norm{f_\nu}^k_{k}\right)>0.
% 	\end{align*}
% 	An exercise in differential calculus gives $\sup_{x\in\R_+} kx^{k-1}\Big(\eta - \lambda x\Big) = \eta^k\left(\frac{k-1}{\lambda k}\right)^{k-1} =:c$,
% 	and we write $c_\epsilon:= c+\epsilon$, for any $\epsilon>0.$
% 	This implies 
% 	that for all $X_s\ge 0$ and $\epsilon>0$, 
% 	\begin{align*}
% 		k X_s^{k-1}\left(
% 		\eta + \frac{1}{2}\left(-c_0 + \frac{k-1}{2} \kappa_4 c_\nu^2 
% 		+ \frac{k-1}{k}+ \norm{f_\mu}_{1} + \frac{C_k}{k} \norm{f_\nu}^k_{k} \right)
% 		 X_s \right) < c_\epsilon,
% 	\end{align*}
% 	from which we can get a bound for the integrand of the first integral in \eqref{equation/1/proofs/1/stationarity/pqUI/E(t)}:
% 	\begin{align*}
% 		&k X_s^{k-1}
% 		\left(\eta+ \left( - c_0 + \frac{k-1}{2} \kappa_4 c_\nu ^2 \right) X_s \right)
% 		\\
% 		&\hspace{2cm}< c_\epsilon - \frac{k}{2}\left(c_0 - \frac{k-1}{2} \kappa_4 c_\nu^2 
% 		+ \frac{k-1}{k}+ \norm{f_\mu}_{1} + \frac{C_k}{k} \norm{f_\nu}^k_{k} \right) X_s^{k}.
% 		\numberthis\label{equation/1/proofs/1/stationarity/pqUI/bound_on_eta_term}
% 	\end{align*}
% 	For the second integral in \eqref{equation/1/proofs/1/stationarity/pqUI/E(t)},  Lemma \ref{lemma/1/stationarity/cross} gives the bound
% 	\begin{align*}
% 		&k\Em\left[X_s^{k-1} \Xi(X)_s\right]
% 		\le 
% 		(k-1) \Big(1+ \norm{f_\mu}_{1}\Big)\Em[X_s^{k}]
% 		+\Big(\norm{f_\mu}_{1} + C_k \norm{f_\nu}^k_{k}\Big)\sup_{u\le s}\Em\left[X_u ^2\right].
% 	\end{align*}
% 	Combining this with \eqref{equation/1/proofs/1/stationarity/pqUI/E(t)} and \eqref{equation/1/proofs/1/stationarity/pqUI/bound_on_eta_term} 
% 	and writing $\bar E(s) = \sup_{u\le s} E(u)$, we have
% 	\begin{align*}
% 		E(t)&\le E(0)
% 		- \lambda_1
% 		\int_0^t E(s) ds
% 		 +  \int_0^t\left( c_\epsilon+ \lambda_2\bar E(s)\right) ds.
% 	\end{align*}
% 	where $\lambda_2 = \norm{f_\mu}_{1} + C_k \norm{f_\nu}^k_{k}$, and
% 	\begin{align*}
% 		\lambda_1:& = 
% 		\frac{k}{2}\left(c_0 - \frac{k-1}{2} \kappa_4 c_\nu^2 
% 		+ \frac{k-1}{k}+ \norm{f_\mu}_{1} + \frac{C_k}{k} \norm{f_\nu}^k_{k} \right)
% 		- (k-1) \Big(1+ \norm{f_\mu}_{1}\Big),
% 	\end{align*}
% 	which gives
% 	\begin{align*}
% 		\lambda_1 - \lambda_2 
% 		& = \frac{k}{2} \lambda>0,
% 	\end{align*}
% 	by our assumed condition \eqref{equation/1/stationarity/pqUIcondition}, i.e., $\lambda_1>\lambda_2$.
% 	By Lemma \ref{lemma/1/stationarity/ItoNisio} (\ref{lemma/1/stationarity/ItoNisio/1}), 
% 	\begin{align*}
% 		E(t)\le  E(0) + \int_0^t e^{-\lambda_1(t-s)}  \left(c_\epsilon+\lambda_2\bar E(s)\right) ds. 
% 		\numberthis\label{equation/1/proofs/1/stationarity/pqUI/E(t)afterfirstGronwall}
% 	\end{align*}
% 	Since $\bar E$ is non-decreasing, a quick integration by parts shows that the integral in \eqref{equation/1/proofs/1/stationarity/pqUI/E(t)afterfirstGronwall} is non-decreasing with respect to $t$. Hence 
% 	\begin{align*}
% 		\bar E(t) = \sup_{u\in [-p,t]} E(u) 
% 		& \le E(0) + \sup_{u\in [-p,t]} \int_0^u e^{-\lambda_1(u-s)}\left(c_\epsilon+\lambda_2\bar E(s)\right) ds
% 		   \\
% 		& = \Em[X(0)^k] + c_\epsilon \frac{1-e^{-\lambda_1 t}}{\lambda_1}
% 		+ \lambda_2 \int_0^t e^{-\lambda_1(t-s)} \bar E(s)ds.
% 	\end{align*}
% 	By Lemma \ref{lemma/1/stationarity/ItoNisio} (\ref{lemma/1/stationarity/ItoNisio/2}), since $\lambda_1>\lambda_2>0$,
% 	\begin{align*}
% 		\sup_{u\in[-p,t]} \Em[X_u ^{k}]  & 
% 		\le \left(\Em[X(0)^k] + c_\epsilon \frac{1-e^{-\lambda_1 t}}{\lambda_1}\right)
% 		\frac{\lambda_1 }{\lambda_1 - \lambda_2} <\infty.
% 	\end{align*}

% 	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 	\vspace{1.2mm}\pf{(\ref{theorem/1/stationarity/Lk p0}).} 
% 	Fix $\epsilon>0, k\ge 1$. Similar to the proof of Theorem \ref{theorem/1/stationarity/moment bound} (\ref{theorem/1/stationarity/Lk pq}), applying It\^o's Lemma to $x\mapsto x^{k+\epsilon}$ yields
% 	\begin{align*}
% 		E(t)&= E(0) 
% 		+(k+\epsilon)\Em\left[ \int_0^t X_s^{k-1+\epsilon}
% 		 \left( \eta+ \left( \frac{k-1}{2} \kappa_4 c_\nu ^2 - c_0\right) X_s \right) ds\right]
% 		   \\
% 		&  + (k+\epsilon)\Em\left[
% 		\int_0^t X_s^{k-1+\epsilon} \left(\int_{-p}^0 f(u)X(s+u) du \right)  
% 		ds\right]
% 		%%
% 		+\frac{(k+\epsilon)\epsilon }{2}\kappa_4 c_\nu^2\Em\left[\int_0^t
% 		 X_s^{k+\epsilon}ds \right].
% 		\numberthis\label{equation/1/proofs/1/stationarity/p0UI/E(t)}
% 	\end{align*}
% 	Similar to the proof of part (\ref{theorem/1/stationarity/Lk pq}), we observe that \eqref{equation/1/moments/p0UIcondition} gives
% 	\begin{align*}
% 		\lambda:= \frac{1}{2}\left(c_0 - \frac{k-1}{2} \kappa_4 c_\nu^2  - \norm{f_\mu}_{1}  \right)>0,
% 	\end{align*}
% 	which implies that for all $X_s\ge 0$ and $\epsilon>0$, 
% 	\begin{align*}
% 		(k+\epsilon)X_s^{k-1+\epsilon}\left(\eta + \frac{1}{2}\left(-c_0+\frac{k-1}{2}\kappa_4 c_\nu^2 + \norm{f_\mu}_{1}\right) X_s \right) < c_\epsilon,
% 	\end{align*}
% 	where $c_\epsilon := \epsilon +\eta^{k+\epsilon} \left(\frac{k+\epsilon -1}{\lambda(k+\epsilon)}\right)^{k+\epsilon-1}$.
% 	Rearranging, we have a bound for the integrand:
% 	\begin{align*}
% 		&(k+\epsilon)X_s^{k-1+\epsilon}
% 		\left(\eta+ \left( - c_0 + \frac{k-1}{2} \kappa_4 c_\nu ^2 \right) X_s \right)
% 		\\
% 		&\hspace{2cm} 
% 		< c_\epsilon - \frac{(k+\epsilon)}{2}\left(c_0 - \frac{k-1}{2} \kappa_4 c_\nu^2 + \norm{f_\mu}_{1}\right) X_s^{k+\epsilon}.
% 		\numberthis\label{equation/1/proofs/1/stationarity/p0UI/bound_on_eta_term}
% 	\end{align*}
% 	For second integral in \eqref{equation/1/proofs/1/stationarity/p0UI/E(t)}, Lemma \ref{lemma/1/stationarity/cross} gives
% 	\begin{align*}
% 		&(k+\epsilon)\Em \left[X_s^{k-1+\epsilon} \int_{-p}^0 f(u) X(s+u) du\right]
% 		\le  (k-1+\epsilon)\norm{f_\mu}_{1} E(s)
% 		+\norm{f_\mu}_{1}\bar E(s) .
% 		\numberthis\label{equation/1/proofs/1/stationarity/p0UI/bound_on_delay_integral}
% 	\end{align*}
% 	Combining \eqref{equation/1/proofs/1/stationarity/p0UI/E(t)}, \eqref{equation/1/proofs/1/stationarity/p0UI/bound_on_eta_term} and \eqref{equation/1/proofs/1/stationarity/p0UI/bound_on_delay_integral}, $E(t)$ can be bounded by
% 	\begin{align*}
% 		E(t)&\le E(0)
% 		- \lambda_1
% 		\int_0^t E(s) ds
% 		 +  \int_0^t\left( c_\epsilon+ \lambda_2\bar E(s)\right) ds.
% 	\end{align*}
% 	where  $\lambda_2 = \norm{f_\mu}_{1}$, and
% 	\begin{align*}
% 		\lambda_1:& = 
% 		\frac{k+\epsilon}{2}\left(c_0 - \frac{k-1}{2} \kappa_4 c_\nu^2 
% 		+\norm{f_\mu}_{1} \right) - (k-1+\epsilon)\norm{f_\mu}_{1} - \frac{(k+\epsilon)\epsilon}{2}\kappa_4 c_\nu^2,
% 	\end{align*}
% 	which gives
% 	\begin{align*}
% 		\lambda_1- \lambda_2& = 
% 		\frac{k+\epsilon}{2}\left(c_0 - \frac{k-1}{2} \kappa_4 c_\nu^2 
% 		-\norm{f_\mu}_{1} - \epsilon\kappa_4 c_\nu^2\right). 
% 	\end{align*}
% 	By our assumed condition \eqref{equation/1/moments/p0UIcondition}, there exists a small enough $\epsilon>0$ such that $\lambda_1> \lambda_2 >0$. The rest of the proof is identical to the proof of Theorem \ref{theorem/1/stationarity/moment bound} (\ref{theorem/1/stationarity/Lk pq}).
% \end{proof}

==> WIP/WIP_SDE.tex <==
%!TEX root = ../main.tex
\subsection{Writing the process as a SDE}
	\subsubsection{Kernel that arises from exchanging the double integral}
	For $t>0$, we start with the process
	\begin{align*}
		X(t) = \theta(t) + \int_{[-p,0]} \int_{[u, t+u]} X(s) ds \mu(du) +\int_{[-q,0]} \int_{(u, t+u]} X(s-) dS(s) \nu(du) .
	\end{align*}
	Exchanging the order of integration in the $ds$ integral, we have
	\begin{align*}
	\int_{[-p,0]} \int_{[u, t+u]} X(s) ds \mu(du) 
			& = \int_{[-p,0]} \int_{[0,t]} X(s+u) ds  \mu(du)
			\\& =  
		\int_{[0,t]} \int_{[-p, 0]} X(s+u)  \mu(du) ds.
	\end{align*}
	Recalling $\nu(\cdot) = c_\nu\delta_0(\cdot) + \int_{\cdot}f_\nu (u)\ind_{[-q,0]}(u)  du$, the second integral can be written as
	\begin{align*}
		\int_{[-q,0]} \int_{(u, t+u]} X(s-) dS(s) \nu(du)
		& =  c_\nu\int_{(0, t]} X(s-) dS(s) + \int_{[-q,0]} \left(\int_{(u, t+u]} X(s-) dS(s)\right)f_\nu(u)du.
		\label{eq_I_2}\numberthis
	\end{align*}
	The second integral above corresponds to the region plotted in Figure \ref{fig_region_of_int} ($r=q$ here)
	\begin{figure}[H]
		\centering
		\caption{The kernel $F$}
		\begin{subfigure}{.5\textwidth}
			\centering
			\includegraphics[width=1\textwidth]{WIP/RegionCopy}
			\caption{Region of integration}
			\label{fig_region_of_int}
		\end{subfigure}%
		\begin{subfigure}{.5\textwidth}
			\centering
			\includegraphics[width=1\textwidth]{WIP/Kernel}
			\caption{Kernel $F$}
			\label{fig_kernel}
		\end{subfigure}
	\end{figure}
	\noindent where the bottom line $\{(-r,-r)+\gamma(1,1) , \gamma\in [0,r]\} $ is not included. 
	Therefore, 
	\begin{align*}
		\int_{[-q,0]} \left(\int_{(u, t+u]} X(s-) dS(s)\right)f_\nu(u)du&=
		\int_{(-q,t]} \left(\int \ind_{[-q,0]}(u) \ind_{(u,t+u]}(s)  X(s-) f_\nu(u)du \right) dS(s)
			\\
		& = \int_{(-q,t]} X(s-) \left(\int \ind_{[-q,0]}(u) \ind_{[s-t,s)}(u)   f_\nu(u)du \right) dS(s)
		   \\
		& = {\int_{(-q,t]} F(t,s) X(s-)   dS(s) },
	\end{align*}
	where the kernel $F$, plotted in \ref{fig_kernel}, is given by 
	\begin{align*}
		F(t,s) :& =  \int_{[-q,0]\cap [s-t,s)} f_\nu(u) du 
		= \int_{[-q\vee (s-t), s\wedge 0]} f_\nu(u) du.
		\label{eq_Kernel_in_I_2}\numberthis
	\end{align*}
	The following proposition collects some properties of the kernel $F$.
	\begin{proposition} \label{proposition:kernel}The kernel $F:\Rm\times\Rm\to\Rm_+$ defined in \eqref{eq_Kernel_in_I_2}
	% \begin{align*}
	%  	F(t,s):= \int_{[-q,0]\cap [s-t,s]} f_\nu(u) du 
	% 	= \int_{[-q\vee (s-t), s\wedge 0]} f_\nu(u) du
	% \end{align*} 
	satisfies the following.
	\begin{enumerate}[(i).]
		\item \label{prop:Kernel_zero} $F$ is constantly zero if $(t,s)\notin (0,\infty)\times(-q,t)$, 
			i.e., if $t\le 0$ or $s\in (-q, t)^\mathsf{c}$. As an immediate consequence,
			\begin{align*}
				\int_{(-q,t]} F(t,s) X(s-)   dS(s) = \int_{\Rm} F(t,s) X(s-)   dS(s).
			\end{align*}
		
		Furthermore, for $(t,s) \in (s+q, \infty)\times(0,\infty)$, $F$ is a constant equal to its supremum
		\begin{align*}
			F^* := \sup_{t,s\in\Rm}F(t,s) = \int_{[-q,0]} f_\nu(u) du<\infty.
		\end{align*}
		\item \label{prop:Kernel_derivative}$F$ is Lipschitz continuous on $\Rm^2$. Furthermore, for every $s\in\Rm$, $t\mapsto F(t,s)$ is a.e. differentiable except at $t=s\vee 0 $ and $t= s+q$. The derivative is given by (a.e.)
		\begin{align*}
			\frac{d}{dt}F(t,s) 
			& = f_\nu(s-t) \ind_{[s\vee0, s+q]}(t).\numberthis\label{eq_derivative_of_kenel}
		\end{align*}
	\end{enumerate}
	\begin{proof}
		(\ref{prop:Kernel_zero}) is immediate from the definition of $F$. 
		(\ref{prop:Kernel_derivative}). Rewrite
		\begin{align*}
			F(t,s) 
				% & = \int_{\Rm} \ind_{[s-t,\infty)}(u)f_{\nu}(u)\ind_{[-q,s\vee0]}(u)
				   % \\
				& = \int_{\Rm} \ind_{[s-t,s)}(u)f_{\nu}(u)\ind_{[-q,0]}(u).
		\end{align*}
		For any $(t_2, s_2)$ and $(t_1,s_1)\in\Rm^2$, we have
		\begin{align*}
			|F(t_2,s_2) - F(t_1, s_1)| 
			& \le |F(t_2,s_2) - F(t_1, s_2)|  + |F(t_1,s_2) - F(t_1, s_1)| 
			   \\
			& \le \int_{\Rm} \left|\ind_{[s_2-t_2, s_2]}(u) - \ind_{[s_2-t_1, s_2]}(u)\right| f_{\nu}(u)\ind_{[-q,0]}(u) du
				\\
			&\quad + \int_{\Rm} \left|\ind_{[s_2-t_1, s_2]}(u) - \ind_{[s_1-t_1, s_1]}(u)\right| f_{\nu}(u)\ind_{[-q,0]}(u) du
			   \\
			& \le \left(\sup_{u\in [-q,0]}f_\nu(u)\right) 
				\left(|t_2-t_1| + |s_2-s_1|+|t_2-t_1|\right) 
				   \\
				& \le 2\left(\sup_{u\in [-q,0]}f_\nu(u)\right) \Big|(t_2,s_2) - (t_1,s_1)\Big|_{\Rm^2},
		\end{align*}
		i.e., $F$ is Lipschitz continuous on $\Rm^2$.

		Furthermore, the integrand of $F$ is independent of $t$ whenever $s-t>s\wedge 0$, i.e. $t< s\vee 0$, or $s-t<-q$, i.e., $t>s+q$, and hence $t\mapsto F(t,s)$ is constant on these regions and the derivative is zero. On $t\in (s\vee0, s+q)$, we have
		\begin{align*}
			F(t,s) = \int^{s\wedge0}_{s-t} f_\nu(u) du,
		\end{align*}
		and by the Fundamental Theorem of Calculus, $t \mapsto F(t,s)$ is continuously differentiable and
		\begin{align*}
			\frac{d}{dt}F(t,s) = f_\nu(s-t)
		\end{align*}
		in the region $t\in (s\vee0, s+q)$.
	\end{proof}
	\end{proposition}    

	Now we study the integrala
	\begin{align*}
		I(t) = \int_{\Rm} F(t,s) X(s-)   dS(s) 
	\end{align*}
	in more detail. Since for almost every $\eta$, $S$ is a function of finite variation, we will fix such an  $\eta$ and treat $I(t,\eta)$ as a Lebesgue Stieljes integral with respect the function $S(\cdot,\eta)$.

	\begin{proposition} \label{proposition:Kernel_integral}
	The process $I(t)$ defined above satisfies the following.
		\begin{enumerate}[(i).]
			\item The path $t \mapsto I(t) \equiv 0$ for all $t\le 0$ and is and non-decreasing for any $t$.
				\label{prop:KernelIntegral_zero}
			\item \label{prop:KernelIntegral_continuity} For almost every $\eta$, $t\mapsto I(t)$ is locally Lipschitz continuous and hence almost everywhere differentiable, with derivative given by 
			\begin{align*}
				\frac{d}{dt}I(t) & =  \int_{\Rm} f_\nu(u-t) \ind_{[u\vee0, u+q]}(t) X(u-) dS(u)
				   \\
				& = \ind_{(0,\infty)}(t)\int_{(t-q,t]} f_\nu(u-t)  X(u-) dS(u).
			\end{align*}
			Furthermore, for any $t\in(0,\infty)$,
			\begin{align*}
				I(t) & = \int_{(0,t]} \int f_\nu(u-s) X(u-) dS(u) ds.
			\end{align*}
		\end{enumerate}
		\begin{proof}
			\noindent (\ref{prop:KernelIntegral_zero}) is obvious since $F\equiv0$ if $t\le 0$. Monotonicity follows from the fact that $S$ is almost surely non-decreasing, $t\mapsto F(t,s)$ is non-decreasing for each $s$, and $X$ is almost surely positive.

			\noindent (\ref{prop:KernelIntegral_continuity}). 
			With probability one, $S$ is non-decreasing and $X$ is positive. Furthermore, $F(t,s)$ vanishes for $s\notin(-q,t)$. Hence by Proposition \ref{proposition:kernel} (\ref{prop:Kernel_derivative}), for any $t_2, t_1\in\Rm_+$, 
			\begin{align*}
				\left| I(t_2) - I(t_1) \right| & \le 
				\int_{\Rm}\left|F(t_2,s)-F(t_1,s)\right| X(s-) dS(s)
				   \\
				& \le 2 \left(\sup_{u\in[-q,0]} f_\nu (u)\right)\left(\int_{[-q,t_2\wedge t_1]} X(s-) dS(s)\right)|t_2-t_1|.
			\end{align*}
			It follows that $t\mapsto I(t)$ is locally Lipschitz continuous almost surely, since with probability one $X$ is locally bounded and $S$ has finite variation on compacts. 

			For every $t\in\Rm_+$, with probability one, the map $s\mapsto F(\cdot,s)X(s-)$ is in $L^1(\Rm, dS)$ since $X$ is almost surely locally bounded and $s\mapsto F(\cdot,s)$ is supported on a compact set. The (almost everywhere) derivative of $t\mapsto F(t,\cdot)$, defined by \eqref{eq_derivative_of_kenel}, is locally in $L^1(\Rm,  dS)$. By the Fundamental Theorem of Calculus, $t\mapsto I(t)$ is differentiable almost everywhere with derivative
			\begin{align*}
				\frac{d}{dt} I(t) & =  \int_{\Rm} \frac{d}{dt}F(t,u) X(u-) dS(u)
				   \\
				& = \int_{\Rm}f_\nu(u-t) \ind_{[u\vee0, u+q]}(t)  X(u-) dS(u)
				   \\
				& = \int_{[t-q, t]} f_\nu(u-t) X(u-) dS(u)
			\end{align*}
			for every $t>0$. Since the function $f_\nu$ and $f_\mu$ are supported on $[-r,0]$, we can write 
			\begin{align*}
				\int_{[t-q, t]} f_\nu(u-t) X(u-) dS(u)= \int_{\Rm} f_\nu(u-t) X(u-) dS(u).
			\end{align*}
			Since $t \mapsto I(t)$ is Lipschitz and hence absolutely continuous, finally we have
			\begin{align*}
				I(t)  -I(0) = \int_{(0, t]} \frac{d}{dt}I(s) ds,
			\end{align*}
			with $I(0) =0 $ since $F(0,s)\equiv0$.
		\end{proof}
	\end{proposition}
	\begin{lemma}[Differentiation under a Lebesgue integral]
		Let $\Omega$ be a measure space  and $F:\Rm\times \Omega\to \Rm$ be a jointly measurable function that satisfies the following.
		\begin{enumerate}
			\item For almost every $t\in\Rm$, $\eta \mapsto F(t,\eta)$ is in $L^1(\Omega)$.
			\item For almost all $\eta\in\Omega$, $t\mapsto F(t,\eta)$ is absolutely continuous (and hence almost everywhere differentiable).
			\item For almost every $t\in\Rm$, the derivative $\eta \mapsto \del_t F(t,\eta)$ is locally integrable.
		\end{enumerate}
		Then $t \mapsto \int_\Omega F(t,\eta) d \eta$ is an absolutely continuous and for almost every $t\in\Rm$, its derivative exists and is given by
		\begin{align*}
			\frac{d}{dt} \int_{\Omega} f(t, \eta) d \eta = \int_{\Omega} \frac{\del}{\del t}f(t,\eta) d \eta.
		\end{align*}
	\end{lemma}
\subsubsection{SDE representation}
	{\bf Keep in mind that $f$ is supported on $[-r,0]$, $r=p$ or $q$. Thoughout, I'll drop region of integration whenever it's clear, i.e., $\int f(u)=\int_\Rm f(u)=\int_{[-r,0]}f(u)$ and $\int f(u-t)=\int_{\Rm} f(u-t)=\int_{[t-r,t]}f(u-t)$}.

	The process we're interested in - it can be written in several ways
	\begin{align*}
		X(t)
		& = \theta(t) + \int_{[0,t]} \int_{[-p, 0]} X(s+u)  \mu(du) ds 
			+ c_\nu \int_{(0,t]} X(s-) dS(s) + \int_{(-q,t]} F(t,s) X(s-)   dS(s)
		   \\
		& = \theta(t) -c_\mu\int_{0}^t X(s) ds 
			+ \int_0^t \int f_\mu(u-s)X(u) duds 
			   \\
			& \quad
			+ c_\nu \int_{0+}^t X(s-) dS(s) 
			+ \int_{(-q,t]}F(t,s)X(s-)dS(s) ,
	\end{align*}
	where the properties of $F$ and of the last integral are collected in Prositions \ref{proposition:kernel} and \ref{proposition:Kernel_integral}.
	By Proposition \ref{proposition:Kernel_integral} (\ref{prop:KernelIntegral_continuity}),
	\begin{align*}
		\int_{(-q,t]} F(t,s) X(s-) dS(s) 
		& =  \int_{(0,t]} \int f_\nu(u -s) X(u-)dS(u) ds .
	\end{align*}
 	Combining these, could express $X$ as the solution of the differential equation
	\begin{align*}
		dX(t) & =  \left(\eta + \int f_\mu(u)X(t+u)\mu(du) + \int f_\nu(u -t) X(u-)dS(u)\right) dt
		+ c_\nu X(t-)  dS(t)
		\\	
		& =  \left(\eta -c_\mu X(t)+ \int f_\mu(u-t)X(u)du + \int f_\nu(u -t) X(u-)dS(u)\right) dt
		+ c_\nu X(t-)  dS(t),
	\end{align*}
	where recall $\theta(t):= X(0)+\eta t$, for $t>0$.
	In fact, this is 
	\begin{align*}
		dX(t) = \Big(\eta-c_\mu  X(t) \Big)dt + c_\nu X(t-) dS(t) + \Xi(t) dt,
	\end{align*}
	where the first two terms are exactly what you get in the COGARCH(1,1) and the process
	\begin{align*}
		\Xi(t) :=  \int f_\mu(u-t) X(u) du + \int f_\nu(u-t) X(u-) dS(u),
	\end{align*}
	is called a ``volatility modulated L\'evy driven Volterra (VMLV)'' or more specifically a ``L\'evy semi-stationary process (LSS)'' process in e.g. \cite{Barndorff-NielsenBenthVeraartEtAl2013}. 
	
	\subsubsection{Compensated Poisson measures}
	Denote by $N(dz, dt)$ the Poisson random measure of the L\'evy process $L$. Let $\Pi_L(dz) \otimes dt$  be its compensator and write $\td N(dz,dt) := N(dz,dt) - \Pi_L(dz) \otimes dt$ for the compensated Poisson measure. We have
	\begin{align*}
		\int_0^t c_\nu X(s-) dS(s) & =  \int_{0}^t \int_{\Rm_0} c_\nu X(s-) z^2 N(dz,dt)
		   \\
		& = \int_{0}^t \int_{\Rm_0} c_\nu X(s-) z^2 \td N(dz,dt) 
			+ \int_0^t \int_{\Rm_0} c_\nu X(s-) z^2 \Pi_L(dz) ds
		   \\
		& =c_\nu \int_{0}^t \int_{\Rm_0} X(s-) z^2 \td N(dz,dt) + c_\nu \kappa_2\int_{0}^t X(s) ds,
	\end{align*}
	where $\kappa_n := \int_{\Rm_0} z^n \Pi_L(dz)$.
	Similarly, 
	\begin{align*}
		\int f_\nu(u -t) X(u-)dS(u) & =  \int \int_{\Rm_0 }f_\nu(u -t) X(u-)z^2  N(dz, du) 
		   \\
		& = \int\int_{\Rm_0 } f_\nu(u -t) X(u-)z^2 \td N(dz, du) + \kappa_2 \int f_\nu(u-t) X(u)du
	\end{align*}
	Recall the definitions $c_0 := c_\mu - \kappa_2 c_\nu$ and $f : = f_\mu + \kappa_2 f_\nu$, from here on, we will write
	\begin{align*}
		dX(t)& = \left(\eta - c_\mu X(t)+ \int f_\mu(u-t)X(u)du + \int f_\nu(u -t) X(u-)dS(u)\right) dt
		+ c_\nu X(t-)  dS(t)
		   \\
		& = \left(\eta - c_0 X(t)+ \int f(u-t)X(u)du + \int\int_{\Rm_0} f_\nu(u -t) X(u-)z^2 \td N(dz, du)\right) dt
		   \\
		& \quad
		+ c_\nu \int_{\Rm_0} X(t-)z^2  \td N(dz, dt).
	\end{align*}



==> WIP/WIP_WIP1.tex <==
%!TEX root = ../WIP.tex
\subsection{WIP1}
\subsubsection{Ito's formula for the variance}
	Recall Ito's formula for L\'evy processes \citet*[Theorem 9.4]{DiNunnoOksendalProske2009}:
	\begin{lemma}[Ito's formula]
		Let $X$ be given by 
		\begin{align*}
			dX(t) = \alpha(t) dt + \int_{\Rm_0} \gamma(t,z) \td N(dz,dt)
		\end{align*}
		and $f$ be a continuously differentiable function. Then $f(X(t))$ is a Ito-L\'evy process with 
		\begin{align*}
			df(X(t)) & =
			\alpha(t) f'(X(t)) dt
			   \\
			& \quad 
			+ \int_{\Rm_0} \Big(f(X(t)+ \gamma(t,z)) - f(X(t)) - \gamma(t, z)f'(X(t))\Big)\nu(dz) dt
			   \\
			& \quad 
			+ \int_{\Rm_0} \Big(f(X(t-)+\gamma(t,z)) - f(X(t-))\Big) \td N(dz,dt).
		\end{align*}
	\end{lemma}
	\noindent By identifying $f(x) = x^2$ and $\nu=\Pi_L$, we have
	\begin{align*}
		X(t)^2- X(0)^2 & =  2 \int_0^t X(s)\alpha(s) ds +\int_0^t \int_{\Rm_0} \gamma(s,z)^2 \Pi_L(dz) ds 
		   \\
		& \quad
		+ \int_0^t\int_{\Rm_0}	\Big(\gamma(s,z)^2 + 2 X(s-) \gamma(s,z)\Big) \td N(dz,ds).
	\end{align*} 
	Identifying $\gamma(s, z) = c_\nu X(s-) z^2$ and 
	\begin{align*}
		\alpha(s) = \eta - c_0 X(s)+ \int f(u-s)X(u)du + \int\int_{\Rm_0} f_\nu(u -s) X(u-)z^2 \td N(dz, du),
	\end{align*}
	we have
	\begin{align*}
		2\int_0^t X(s)\alpha(s) ds  & =  2\eta \int_{0}^{t} X(s) ds - 2c_0 \int_0^t X(s)^2 ds
		\\
		& \quad + 2\int_0^t X(s) \left(\int f(u-s) X(u)du\right) ds
		   \\
		& \quad + 2 \int_0^t X(s) \left(\int\int_{\Rm_0} f_\nu(u-s) X(u-) z^2 \td N(dz, du)\right) ds.
	\end{align*}
	which has expectation given by CAREFUL HERE
	\begin{align*}
		&\Em\left(2\int_0^t X(s)\alpha(s)  ds \right)
			\\
		& =  2 \left(\eta \int_0^t \Em (X(s)) ds - c_0\int_0^t \Em (X(s)^2) ds 
		+ \int_0^t \int f(u-s) \Em(X(s)X(u)) du ds\right)
		   \\
		& \quad+2 \int_0^t \Em\left(  X(s) \left(\int\int_{\Rm_0} f_\nu(u-s) X(u-) z^2 \td N(dz, du)\right)
			     \right) ds
	\end{align*}
	The second term in the Ito formula:
	\begin{align*}
		&\int_0^t\int_{\Rm_0} \gamma(s,z)^2  \Pi_L(dz) ds
		 =\int_0^t \int_{\Rm_0}  c_\nu^2 X(s)^2 z^4 \ \Pi_L(dz) ds
		 = \kappa_4 c_\nu^2  \int_0^t X(s)^2 ds.
	\end{align*}
	Putting all these together and noting $\int d\td N$ has zero expectation, we an expression for the second moment of $X$:
	\begin{align*}
		\Em\left(X(t)^2\right) & = \Em(X(0))^2 + 2 \eta \int_0^t \Em (X(s)) ds 
		+ (\kappa_4 c_\nu^2 - 2c_0)\int_0^t \Em (X(s)^2) ds 
		   \\
		& \quad + 2\int_0^t \int f(u-s) \Em(X(s)X(u)) du ds
			\\
		&\quad
		+2 \int_0^t \Em\left(  X(s) \left(\int\int_{\Rm_0} f_\nu(u-s) X(u-) z^2 \td N(dz, du)\right)
			     \right) ds.
	\end{align*}
	\subsubsection{Malliavin calculus}
	Using the duality between the Malliavin derivative and the Skorohod integral (Theorem 12.10 \cite{DiNunnoOksendalProske2009}), we could write
	\begin{align*}
		\Em\left(  X(s) \left(\int\int_{\Rm_0} f_\nu(u-s) X(u-) z^2 \td N(dz, du)\right)\right)
		& = \Em \int \int_{\Rm_0} D_{u,z}X(s) X(u-) f_\nu(u-s) z^2  \nu(dz) du,
	\end{align*}
	but I doubt we could work out what 
	\begin{align*}
		\Em\left(X(u-)D_{u,z}X(s) \right)
	\end{align*}
	is - I doubt I can get an explicit formula for the derivative. Chaos expansion of $X(u)=X(u,z)$: there exists a sequence $f_n(\cdot, u,z)\in \td L^2\left(\left(dt\times d\nu\right)^n\right)$ such that 
	\begin{align*}
		X(u) = \sum_{n=0}^{\infty} I_n(f_n(\cdot, u,z)),
	\end{align*}
	where $I_n$ denotes the $n$-th iterated integral against $\td N(dz,dt)$.
	Similarly, write
	\begin{align*}
		X(s) = \sum_{n=0}^{\infty} I_n(f_n(\cdot, s,z)),
	\end{align*}
	(assuming differentiability or whatever that you need), which gives
	\begin{align*}
		D_{u,z}X(s) = \sum_{n=1}^{\infty} nI_{n-1}(f_n(\cdot,u,z, s,z)).
	\end{align*}
	The isometry then gives
	\begin{align*}
		\Em\left[X(u-)D_{u,z}X(s)\right] 
		& = \Em\left[\sum_{n=0}^{\infty} I_n(f_n(\cdot, u,z))
			\sum_{n=1}^{\infty} nI_{n-1}(f_n(\cdot,u,z, s,z)).\right]
			   \\
		& = \Em\left[\sum_{n=0}^{\infty} I_n(f_n(\cdot, u,z))
			\sum_{n=0}^{\infty} (n+1)I_{n}(f_{n+1}(\cdot,u,z, s,z)).\right]
			   \\
		& = \sum_{n=0}^{\infty} (n+1) \int\cdots\int f_n(\cdot,u)f_{n+1}(\cdot,u,s) d\nu dt\cdots d\nu dt
	\end{align*}
	doesn't look very promising.

	
	\subsubsection{Covariance by Ito, q=0}
	Write
	\begin{align*}
		dY(T) & = 
		\ind_{[0,t]}(T)\left(\Big( \eta- c_0 X(T) + \int f(u-T) X(u)du \Big)dT
						+ \int_{\Rm_0}c_\nu X(T-)z^2 \td N(dz,dT)\right)
		   \\
		& = dX(t\wedge T)
		   \\
		dY_h(T) & = 
		\ind_{[0,t+h]}(T)\left(\Big( \eta- c_0 X(T) + \int f(u-T) X(u)du \Big)dT
						+ \int_{\Rm_0}c_\nu X(T-)z^2 \td N(dz,dT)\right)
		   \\
		& =  dX((t+h)\wedge T)
	\end{align*}
	so that $Y(T) = X(t)$ for all $T>t$ and $Y_h(T)= X(t+h)$ for all $T>t+h$. By Ito's product formula, (Example 9.7, p.167, \cite{DiNunnoOksendalProske2009})
	\begin{align*}
		d(Y(T)Y_h(T)) = Y(T-) dY_h(T)+  Y_h(t-) dY(t) 
		+\ind_{[0,t\wedge(t+h)]}(T) \int_{\Rm_0} c_\nu^2 X(T-)^2 z^4 N(dz,dT).
	\end{align*}
	Fixing $T>t+h$, first term becomes
	\begin{align*}
		&\int_0^T Y(s-)dY_h(s)  =  \int_0^T X(t\wedge s) dY_h(s)
		   \\
		& = \int_0^{t+h} X(t\wedge s) \Big( \eta- c_0 X(s) + \int f(u-s) X(u)du \Big)ds
		+\int_0^{t+h}\int_{\Rm_0}  X(t\wedge s) \Big(c_\nu X(s-)z^2\Big) \td N(dz,ds)
		   \\
		& = \int_0^{t} X(s) \Big( \eta- c_0 X(s) + \int f(u-s) X(u)du \Big)ds
		+\int_0^{t}\int_{\Rm_0}  c_\nu X(s-)^2z^2  \td N(dz,ds)
		   \\
		& \quad+\int_t^{t+h} X(t) \Big( \eta- c_0 X(s) + \int f(u-s) X(u)du \Big)ds
		+\int_t^{t+h}\int_{\Rm_0}  X(t) \Big(c_\nu X(s-)z^2\Big) \td N(dz,ds).
	\end{align*}
	Notice here the integrands of the stochastic integrals are adapted. Second term:
	\begin{align*}
		&\int_0^T Y_h(s-)dY(s)  =  \int_0^T X((t+h)\wedge s) dY(s)
		   \\
		& = \int_0^{t} X((t+h)\wedge s) \Big( \eta- c_0 X(s) + \int f(u-s) X(u)du \Big)ds
		+\int_0^{t} \int_{\Rm_0} X((t+h)\wedge s) \Big(c_\nu X(s-)z^2\Big) \td N(dz,ds)
		   \\
		& = \int_0^{t} X(s) \Big( \eta- c_0 X(s) + \int f(u-s) X(u)du \Big)ds
		+\int_0^{t}\int_{\Rm_0}  c_\nu X(s-)^2z^2  \td N(dz,ds).
	\end{align*}
	Taking expectations:
	\begin{align*}
		&\Em(X(t+h)X(t))  =\Em(X(0)X(h))+ c_\nu^2 \kappa_4 \int_0^t \Em(X(s)^2) ds
		   \\
		& \quad+  2 \eta \int_0^t \Em(X(s)) ds - 2c_0\int_0^t \Em(X(s)^2) ds 
		+ 2 \int_0^t \int f(u-s) \Em(X(u)X(s)) du ds
		   \\
		& \quad + \eta h \Em(X(t)) - c_0\int_t^{t+h} \Em(X(t)X(s)) ds 
		+ \int_t^{t+h}\int f(u-s)\Em(X(u)X(t)) du ds.
	\end{align*}
	Recall that the mean is given by
	\begin{align*}
		m_X(t) & =  m_X(0) -c_0 \int_0^t m_X(s) ds + \int_0^t \int f(u-s)m_X(u) du ds
		   \\
		m_X(t+h) & =  m_X(0) -c_0 \int_0^{t+h} m_X(s) ds + \int_0^{t+h} \int f(u-s)m_X(u) du ds.
	\end{align*}
	By a similar product rule, 
	\begin{align*}
		&m_X(t)m_X(t+h)  = m_X(0)m_X(h)
		   \\
		& \quad + 2 \eta\int_0^t m_X(s) ds -2c_0 \int_0^t m_X^2(s) ds 
		+ 2\int_0^t \int f(u-s) m(s)m(u) du ds 
		   \\
		& \quad + \eta h m_X(t) - c_0\int_t^{t+h} m_X(s)m_X(t) ds + \int_t^{t+h}\int f(u-s) X(u)x(t) du ds.
	\end{align*}
	Therefore, denoting $C_X(t,s)=\Cov(X(t),X(s))$ and $V_X(t) = \Var(X(t))$, we have
	\begin{align*}
		C_X(t,t+h) & = C_X(0,h) 
		   \\
		& \quad+ (c_\nu^2 \kappa_4 -2c_0)\int_0^t V_X(s) ds 
		+ c_\nu^2 \kappa_4\int_0^t m_X^2(s) ds 
		+ 2\int_0^t\int f(u-s) C_X(u,s) du ds
		   \\
		& \quad -c_0\int_t^{t+h} C_X(t,s)ds + \int_t^{t+h}\int f(u-s) C_X(t,u) du ds.
	\end{align*}
	Using the formula for the variance derived earlier, we have
	\begin{align*}
		C_X(t,t+h) = C_X(0,h) + V_X(t) - V_X(0)-c_0\int_t^{t+h} C_X(t,s)ds + \int_t^{t+h}\int f(u-s) C_X(t,u) du ds.
	\end{align*}
	Changing variables,
	\begin{align*}
		&C_X(t,t+h) - C_X(0,h) - V_X(t) + V_X(0)  
			\\
		& =  -c_0\int_0^{h} C_X(t,t+s)ds + \int_0^{h}\int_{-p}^0 f(u) C_X(t,t+s+u) du ds
		   \\
		& =  \int_{-p}^0  \int_0^{h} C_X(t,t+s)ds \td\mu(du),
	\end{align*}
	where $\td\mu(du) = -c_0\delta_0(du)+ f(u) du$.
	Again, assuming second order stationarity,
	\begin{align*}
		\gamma_X(h) = \gamma_X(h) + V_X - V_X - c_0 \int_t^{t+h} \gamma_X(t-s) ds 
		+ \int_{t}^{t+h} \int _{[s-p,s]}f(u-s) \gamma_X(t-u)du ds
		\end{align*}
	which gives
	\begin{align*}
		c_0 \int_t^{t+h} \gamma_X(s-t) ds & = \int_{t}^{t+h}\int_{[s-p,s]} f(u-s) \gamma_X(u-t)du ds
		   \\
		c_0 \int_0^{h} \gamma_X(s) ds& = \int_{t}^{t+h}\int_{[-p,0]} f(u) \gamma_X(u-t+s)du ds.
	\end{align*}
	Differentiating, we have
	\begin{align*}
		c_0 \gamma_X(h) = \int_{-p}^0 f(u) \gamma_X(u+h) du
	\end{align*}
	I'm pretty sure this is incorrect - the only solution to this is the zero solution. Can't figure out where it went wrong though.
	\subsubsection{Another thought for the variance}
	First,
	\begin{align*}
		\int_{(-q,t]} F(t,s)X(s-)dS(s) & = \kappa_2 \int_{-q}^t F(t,s)X(s) ds+
		\int_{(-q,t]} F(t,s)X(s-)d\td S(s)  
		   \\
		& = \kappa_2 \int_{0}^t \int_{s-q}^s f_\nu(s-u) X(u) du ds+
		\int_{(-q,t]} F(t,s)X(s-)d\td S(s) 
	\end{align*}
	and we could write
	\begin{align*}
		X(t) & =  X(0) + \int_0^t\left(\eta - c_0 X(s) +  \int_{s-r}^s f(u-s) X(u)du\right)ds 
		+c_\nu \int_{(0,t]} X(s-)d\td S(s) + \int_{(-q,t]}F(t,s)X(s-)d\td S(s)
		   \\
		& = X(0) + \int_0^t \alpha(s) ds + \int \gamma_1(s) d\td S(s) + \int \gamma_2(s) d\td S(s) 
	\end{align*}
	Computations of $X(t)^2$:
	\begin{align*}
		X(t)^2 = X(0)X(t)+ \int_0^t X(t) \alpha(s) ds + X(t)\int \gamma_1(s) d\td S(s) 
		+ X(t)\int \gamma_2(s) d\td S(s)
	\end{align*}
	term by term: first
	\begin{align*}
		\Em(X(0)X(t))= C_X(0,t)
	\end{align*}
	second
	\begin{align*}
		\Em \left(\int_0^t X(t) \alpha(s) ds\right)
		= \eta t m_X(t) -c_0\int_0^t C_X(t,s)ds + \int_0^t \left(\int f(u-s) C_X(t,u) du\right) ds
	\end{align*}
	third
	\begin{align*}
		&c_\nu X(t)\int_0^t X(s-)d\td S(s)
		   \\
		& = c_\nu X(0)\int_0^t X(s-)d\td S(s)
		   \\
		& \quad +  c_\nu\left(\int_0^t\left(\eta - c_0 X(s) +  \int_{s-r}^s f(u-s) X(u)du\right)ds \right)\left(\int_0^t X(s-)d\td S(s)\right)
		\\&\quad+\left(c_\nu \int_{(0,t]} X(s-)d\td S(s)\right)^2
		   \\
		& \quad + c_\nu\left(\int_{(-q,t]}F(t,s)X(s-)d\td S(s)\right)\left(\int_0^t X(s-)d\td S(s)\right)
	\end{align*}
	with expectation
	\begin{align*}
		\Em \left( c_\nu X(t)\int_0^t X(s-)d\td S(s) \right)= 0 + 0 
		+ c_\nu^2 \kappa_4 \int_0^t \Em(X(s)^2) ds
		+ c_\nu \kappa_4 \int_0^t F(t,s) \Em(X(s)^2) ds.
	\end{align*}
	Last term
	\begin{align*}
		&X(t)\int_{(-q,t]}F(t,s)X(s-)d\td S(s)
		   \\
		& = X(0)\left(\int_{(-q,t]}F(t,s)X(s-)d\td S(s)\right)
		   \\
		& \quad +\left(\int_0^t\left(\eta - c_0 X(s) +  \int_{s-r}^s f(u-s) X(u)du\right)ds \right) 
				\left(\int_{(-q,t]}F(t,s)X(s-)d\td S(s)\right)
		\\&\quad+\left(c_\nu \int_{(0,t]} X(s-)d\td S(s)\right)\left(\int_{(-q,t]}F(t,s)X(s-)d\td S(s)\right)
		   \\
		& \quad + \left(\int_{(-q,t]}F(t,s)X(s-)d\td S(s)\right)^2.
	\end{align*}
	Last two terms in the expression are simple, with expectation
	\begin{align*}
		c_\nu \kappa_4 \int_0^t F(t,s)\Em(X(s)^2) ds + \kappa_4 \int_0^t F(t,s)^2 \Em(X(s)^2) ds.
	\end{align*}
	Write 
	\begin{align*}
		\int_{(-q,t]}F(t,s)X(s-)d\td S(s) = \int_0^t \int_{s-q}^s f_\nu(u-s) X(u-) d\td S(u) ds
	\end{align*}
	We still need 
	\begin{align*}
		&X(0)\left(\int_{(-q,t]}F(t,s)X(s-)d\td S(s)\right)
		\\
		&\quad+\left(\int_0^t\left(\eta - c_0 X(s) +  \int_{s-r}^s f(u-s) X(u)du\right)ds \right) 
				\left(\int_{(-q,t]}F(t,s)X(s-)d\td S(s)\right)
	\end{align*}
	still doesn't solve the problem though. No matter what I do here, can't get around the expected value of the cross termspectral decompositionis there anyway around this problem?


==> WIP/WIP_WIP2.tex <==
%!TEX root = ../WIP.tex
\subsection{WIP2}
	\subsubsection{Process Y} 
	Here we consider the price process, the differenced returns, and the differenced squared returns. The price process
	\begin{align*}
		Y(t) - Y_0=  \int_{0+}^t \rt{X(s-)} dL(s), \quad t> 0
	\end{align*}
	has moments
	\begin{align*}
		\Em [Y(t)] & =  \Em[Y_0],
		   \\
		\Cov(Y(s),Y(t)|Y_0)& = \td \kappa_2 \int_{0}^{s\minn t} m^X(s) ds.
	\end{align*}
	where recall $m^X(t) = \Em[X(t)]$.
	Assuming $X$ satisfies the stationarity conditions, then
	\begin{align*}
		\Cov(Y(s), Y(t)|Y_0)& = (s\minn t)\td \kappa_2 m_X .
	\end{align*}
	Fix $\tau>0$, let $(Y^{(\tau)}(t))_{t> 0}$ be the $\tau$-differenced return process  
	\begin{align*}
		Y^{(\tau)}(t)= Y(t+\tau) - Y(t)  = \int_{t+}^{t+\tau} \rt{X(s-)} dL(s).
	\end{align*}
	Let $h\ge 0$, the moments are given by
	\begin{align*}
		&\Em [Y\d{\tau}(t)]  =  0,
		\qquad\Cov(Y\d{\tau}(t), Y\d{\tau}(t+h))  = 	\td \kappa_2 \int_{t+h}^{t+\tau} m^X(s) ds.
	\end{align*}
	If $X$ is first order stationary, $Y^{(\tau)}$ is second order stationary with
	\begin{align*}
		\Em [Y\d{\tau}(t)] & =  0,\qquad
		\Cov(Y\d{\tau}(t), Y\d{\tau}(t+h))  = \ind_{\{\tau>h\}} (\tau - h) \td\kappa_2m_X.
	\end{align*}
	By It\^o's lemma, we can write the squared differenced returns as
	\begin{align*}
		 Y\d{\tau}(t)^2 
		& =  (Y(t+\tau) - Y(t))^2
		   \\
		& = 2\int_{t+}^{t+\tau} Y(s-) \rt{X(s-)} dL(s) + \int_{t+}^{t+\tau} X(s-) d[L,L](s)
		   \\
		& = \int_{t+}^{t+\tau}\int_{\Rm_0}\left(2Y(s-)\right) \td N (dz,ds)
	\end{align*}
	Similarly,
	\begin{align*}
		Y^{(\tau)}(t)^4 
		& = \int_{t+}^{t+\tau} 4Y(s-)^3 \rt{X(s-)} dL(s) + \int_{t+}^{t+\tau}6 Y(s-)^2 X(s-) d[L,L](s),
	\end{align*}
	which gives
	\begin{align*}
		\Em\left[Y^{(\tau)}(t)^4\right] = 6 \td \kappa_2\int_t^{t+\tau} \Em\left[Y(s)^2X(s)\right] ds
	\end{align*}
	\begin{align*}
		(Y(t)-Y(0))^2 X(t) & =  X(t) \left(\int_{0+}^t \rt{X(s-)} dL(s)\right)^2
		   \\
		& = X(t) \left(2\int_{0+}^{t} Y(s-) \rt{X(s-)} dL(s) + \int_{0}^{t} X(s-) d[L,L](s)\right)
	\end{align*}
	Taking expectation yields
	\begin{align*}
		\Em \left[Y\d{\tau}(t)^2\right] = 
	\end{align*}
	\begin{align*}
		\Em\left[Y^{(\tau)}(t)^2\ Y\d{\tau}(t+h)^2 \right] & =  \Em\left[Y^{(\tau)}(0)^2\ Y\d{\tau}(h)^2 \right]
		   \\
		& = \Em\left[(Y(\tau) - Y(0))^2 \left(
			\int_{h+}^{h+\tau} \rt{X(s-)} dL(s)\right)^2 \right]
	\end{align*}
	

	\subsubsection{Between jumps}
	Recall $\td \kappa_2 = \int_{\Rm_0} z^2 \Pi_L(dz)+ \sigma_L^2$ and $c_0  = c_\mu - \td\kappa_2 c_\nu$. Let $T_0, T_1, \cdots$ be the jump times of the subordinator $S(t) = \td \kappa_2 t + \tilde S(t)$. For each $j\in \N_0$, $X$ follows a deterministic delay equation
	\begin{align*}
		\frac{d}{dt}X(t) = \eta - c_0 X(t) + \int_{-p}^0 f(u) X(t+u) du, \quad t \in (T_j, T_{j+1}),
		\numberthis\label{eq_p0/FDEbetweenjumps}
	\end{align*}
	with initial condition ${X(u), u\in [T_j - p, T_j]}$.
	Let $\cL_X(\xi) = \int_{0}^{\infty} e^{-\xi t} X(s)dt$ be the Laplace transform of $X$. 
	The Laplace transform of a convolution product $(f*g) (t) := \int_0^t f(u) g(t-u) du$ is given by $\cL_f(\xi) \cL_f (\xi)$. Rewriting the delay integral into
	\begin{align*}
		\int_{-p}^0 f(u) X(t+u) du & = \int_{t-p}^t f(u-t) X(u) du
		   \\
		& = \int_0^t  X(u) f(-(t-u))\ind_{[0,p]}(t-u) du
		   \\
		& =  \left(X *		f(-\cdot)\ind_{[0,p]}(\cdot)  \right)(t),
	\end{align*}
	we have
	\begin{align*}
		\cL_{X *		f(-\cdot)\ind_{[0,p]}(\cdot)}(\xi)
		& = \cL_X(\xi) \cL_{f(-\cdot)\ind_{[0,p]}(\cdot)}(\xi)
		   \\
		& = \cL_X(\xi)\int_0^p e^{-\xi t} f(-t) dt
	\end{align*}
	Furthermore, by the properties of the Laplace transform, we have $\cL_{\dot X} =  \cL_X(\xi)/\xi - X(0)$ and $\cL_{\eta} = 1/\xi$. Taking Laplace transforms of both sides of \eqref{eq_p0/FDEbetweenjumps} then yields
	\begin{align*}
		\frac{1}{\xi} \cL_X(\xi) - X(0) = \frac{\eta}{\xi} - c_0 \cL_X(\xi) + \cL_X(\xi)\int_0^p e^{-\xi t} f(-t) dt, 
	\end{align*}
	which gives
	\begin{align*}
		\cL_X(\xi) = \frac{\eta + X(0)\xi  }{1 + \Big(c_0- \int_0^p e^{-\xi t} f(-t) dt\Big)\xi}.
	\end{align*}
	We can then numerically invert the Laplace transform to get the solution. 

	\subsubsection{Convoluted L\'evy Process}
	For $t\ge 0$, denote
	\begin{align*}
		J(t) = \int_{\Rm} \ind_{[t-q,t]}(u) f_\nu(u-t) X(u-) d\td S(u).
	\end{align*}
	Since the function $f$ is of bounded variation on $\Rm_+$ and $\td S$ is c\`adl\`ag and of bounded variation with probability one, $J(t)$ is c\`adl\`ag and of bounded variation and hence a semimartingale.
	For the jumps of this process, 
	for $h>0$, 
	\begin{align*}
		J(t) - J(t-h) & =  \int \ind_{(t-h, t]}(u)f_\nu(u-t)X(u-) d\td S(u)
		    - \int \ind_{(t-q-h, t-q]}(u)f_\nu(u-t+h)X(u-) d\td S(u)
		   \\
		& \quad + \int \ind_{(t-q, t-h]}(u) \Big(f_\nu(u-t) - f_\nu(u-t+h)\Big) X(u-) d\td S(u),
	\end{align*}
	where the integrand is compactly supported and locally bounded, and hence the sup of the integrand is integrable with respect to $d\td S$. Taking $h$ to zero and using Dominated Convergence Theorem,
	\begin{align*}
		\Delta J(t) = J(t) - J(t-) & = 	f_\nu(0) X(t-) \Delta \td S(t) - f_\nu(-q) X(t-q) \Delta\td S(t-q)
	\end{align*}
	\begin{proposition}
		For $t\ge 0$, the jumps of $t\mapsto J(t)$ is indistinguishable from the jumps of 
		\begin{align*}
			\hat J(t):& = f_\nu(0)\int_0^t X(u-)d\td S(u) - f_\nu(-q) \int_0^t X\left((u-q)-\right)d\td S(u-q)
			   \\
			& = f_\nu(0)\int_0^t X(u-)d\td S(u) - f_\nu(-q) \int_{-q}^{t-q} X\left(u-\right)d\td S(u)
			   \\
			& = \int_{-q}^t \Big(f_\nu(0)\ind_{(0,t]}(u) - f_\nu(-q) \ind_{(-q,t-q]}(u) \Big)X(u-)d\td S(u).
		\end{align*}
	\end{proposition}
	Furthermore, for $h>0$ we have
	\begin{align*}
		\frac{J(t) - J(t-h)}{h} & =  \int \left(\frac{\ind_{(0, t]}(u)- \ind_{(0, t-h]}(u)}{h}\right)f_\nu(u-t)X(u-) d\td S(u)
		   \\
		& \quad - \int \left(\frac{\ind_{(0, t-q]}(u)- \ind_{(0, t-q-h]}(u)}{h}\right)f_\nu(u-t+h)X(u-) d\td S(u)
		   \\
		& \quad + \int \ind_{(t-q, t-h]}(u) \left(\frac{f_\nu(u-t) - f_\nu(u-t+h)}{h}\right) X(u-) d\td S(u).
	\end{align*}
	Letting $h\to0$, formally we should have the limit
	\begin{align*}
		\frac{dJ(t)}{dt} & =  \int \delta_t(u) f_\nu(u-t) X(u-) d\td S(u) - \int \delta_{t-q}(u) f_\nu(u-t) X(u-) d\td S(u)
		   \\
		& \quad + \int_{(t-q ,t)} f'_\nu(u-t) X(u-) d\td S(u)
		   \\
		& = f_\nu(0) X(t-) d\td S(t) - f_\nu(-q) X\left((t-q)-\right) d\td S(t-q) + \int_{(t-q ,t)} f'_\nu(u-t) X(u-) d\td S(u),
	\end{align*}
	since $f_\nu$ is differentiable in $(-q,0)$. 




	The process $\td X(t) = X(t) - M_X(t)$ is also a local martingale right? Assuming it is,
	\begin{align*}
		\Em(X(t) J(t)) & =  \Em(X(t)J(t) )
		   \\
		& = \Em(\td X(t) J(t)) + \Em(M_X(t)J(t)),
	\end{align*}
	where the second term is zero since $M_X$ is deterministic.
	The jumps of $\td X$ is given by
	\begin{align*}
		\Delta \td X(t) = c_\nu X(t-) \Delta S(t),
	\end{align*}
	(needs proof as well) so we have
	\begin{align*}
		\Em(\td X(t) J(t)) & = \Em [\td X, J](t)
		   \\
		& = \Em \sum_{u\le t}\Delta \td X(u)\Delta J(u)
		   \\
		& = \sum_{u\le t} \left\{c_\nu f_\nu(0) X(u-)^2 (\Delta \td S(u) )^2 
				- c_\nu f_\nu(-q) X(u-)X(u-q) \Delta \td S(u)\td S(u-q)\right\}
				   \\
		& = c_\nu f_\nu(0) \int_0^t\int_{\Rm_0} X(t-)^2 z^4 \td N(dz,dt)
		- c_\nu f_\nu(-q) \int_0^t \int_{\Rm_0} X(u-)X(u-q) z_1 z_2 \td N()
	\end{align*}
	
	\subsubsection{Variation of constants}






































	

==> WIP/WIP_WIP3.tex <==
%!TEX root = ../WIP.tex
\subsection{WIP}
\subsubsection{Ito's formula for the variance}
	Recall Ito's formula for L\'evy processes \citet*[Theorem 9.4]{DiNunnoOksendalProske2009}:
	\begin{lemma}[Ito's formula]
		Let $X$ be given by 
		\begin{align*}
			dX(t) = \alpha(t) dt + \int_{\Rm_0} \gamma(t,z) \td N(dz,dt)
		\end{align*}
		and $f$ be a continuously differentiable function. Then $f(X(t))$ is a Ito-L\'evy process with 
		\begin{align*}
			df(X(t)) & =
			\alpha(t) f'(X(t)) dt
			   \\
			& \quad 
			+ \int_{\Rm_0} \Big(f(X(t)+ \gamma(t,z)) - f(X(t)) - \gamma(t, z)f'(X(t))\Big)\nu(dz) dt
			   \\
			& \quad 
			+ \int_{\Rm_0} \Big(f(X(t-)+\gamma(t,z)) - f(X(t-))\Big) \td N(dz,dt).
		\end{align*}
	\end{lemma}
	\noindent By identifying $f(x) = x^2$ and $\nu=\Pi_L$, we have
	\begin{align*}
		X(t)^2- X(0)^2 & =  2 \int_0^t X(s)\alpha(s) ds +\int_0^t \int_{\Rm_0} \gamma(s,z)^2 \Pi_L(dz) ds 
		   \\
		& \quad
		+ \int_0^t\int_{\Rm_0}	\Big(\gamma(s,z)^2 + 2 X(s-) \gamma(s,z)\Big) \td N(dz,ds).
	\end{align*} 
	Identifying $\gamma(s, z) = c_\nu X(s-) z^2$ and 
	\begin{align*}
		\alpha(s) = \eta - c_0 X(s)+ \int f(u-s)X(u)du + \int\int_{\Rm_0} f_\nu(u -s) X(u-)z^2 \td N(dz, du),
	\end{align*}
	we have
	\begin{align*}
		2\int_0^t X(s)\alpha(s) ds  & =  2\eta \int_{0}^{t} X(s) ds - 2c_0 \int_0^t X(s)^2 ds
		\\
		& \quad + 2\int_0^t X(s) \left(\int f(u-s) X(u)du\right) ds
		   \\
		& \quad + 2 \int_0^t X(s) \left(\int\int_{\Rm_0} f_\nu(u-s) X(u-) z^2 \td N(dz, du)\right) ds.
	\end{align*}
	which has expectation given by CAREFUL HERE
	\begin{align*}
		&\Em\left(2\int_0^t X(s)\alpha(s)  ds \right)
			\\
		& =  2 \left(\eta \int_0^t \Em (X(s)) ds - c_0\int_0^t \Em (X(s)^2) ds 
		+ \int_0^t \int f(u-s) \Em(X(s)X(u)) du ds\right)
		   \\
		& \quad+2 \int_0^t \Em\left(  X(s) \left(\int\int_{\Rm_0} f_\nu(u-s) X(u-) z^2 \td N(dz, du)\right)
			     \right) ds
	\end{align*}
	The second term in the Ito formula:
	\begin{align*}
		&\int_0^t\int_{\Rm_0} \gamma(s,z)^2  \Pi_L(dz) ds
		 =\int_0^t \int_{\Rm_0}  c_\nu^2 X(s)^2 z^4 \ \Pi_L(dz) ds
		 = \kappa_4 c_\nu^2  \int_0^t X(s)^2 ds.
	\end{align*}
	Putting all these together and noting $\int d\td N$ has zero expectation, we an expression for the second moment of $X$:
	\begin{align*}
		\Em\left(X(t)^2\right) & = \Em(X(0))^2 + 2 \eta \int_0^t \Em (X(s)) ds 
		+ (\kappa_4 c_\nu^2 - 2c_0)\int_0^t \Em (X(s)^2) ds 
		   \\
		& \quad + 2\int_0^t \int f(u-s) \Em(X(s)X(u)) du ds
			\\
		&\quad
		+2 \int_0^t \Em\left(  X(s) \left(\int\int_{\Rm_0} f_\nu(u-s) X(u-) z^2 \td N(dz, du)\right)
			     \right) ds.
	\end{align*}
	\subsubsection{Malliavin calculus}
	Using the duality between the Malliavin derivative and the Skorohod integral (Theorem 12.10 \cite{DiNunnoOksendalProske2009}), we could write
	\begin{align*}
		\Em\left(  X(s) \left(\int\int_{\Rm_0} f_\nu(u-s) X(u-) z^2 \td N(dz, du)\right)\right)
		& = \Em \int \int_{\Rm_0} D_{u,z}X(s) X(u-) f_\nu(u-s) z^2  \nu(dz) du,
	\end{align*}
	but I doubt we could work out what 
	\begin{align*}
		\Em\left(X(u-)D_{u,z}X(s) \right)
	\end{align*}
	is - I doubt I can get an explicit formula for the derivative. Chaos expansion of $X(u)=X(u,z)$: there exists a sequence $f_n(\cdot, u,z)\in \td L^2\left(\left(dt\times d\nu\right)^n\right)$ such that 
	\begin{align*}
		X(u) = \sum_{n=0}^{\infty} I_n(f_n(\cdot, u,z)),
	\end{align*}
	where $I_n$ denotes the $n$-th iterated integral against $\td N(dz,dt)$.
	Similarly, write
	\begin{align*}
		X(s) = \sum_{n=0}^{\infty} I_n(f_n(\cdot, s,z)),
	\end{align*}
	(assuming differentiability or whatever that you need), which gives
	\begin{align*}
		D_{u,z}X(s) = \sum_{n=1}^{\infty} nI_{n-1}(f_n(\cdot,u,z, s,z)).
	\end{align*}
	The isometry then gives
	\begin{align*}
		\Em\left[X(u-)D_{u,z}X(s)\right] 
		& = \Em\left[\sum_{n=0}^{\infty} I_n(f_n(\cdot, u,z))
			\sum_{n=1}^{\infty} nI_{n-1}(f_n(\cdot,u,z, s,z)).\right]
			   \\
		& = \Em\left[\sum_{n=0}^{\infty} I_n(f_n(\cdot, u,z))
			\sum_{n=0}^{\infty} (n+1)I_{n}(f_{n+1}(\cdot,u,z, s,z)).\right]
			   \\
		& = \sum_{n=0}^{\infty} (n+1) \int\cdots\int f_n(\cdot,u)f_{n+1}(\cdot,u,s) d\nu dt\cdots d\nu dt
	\end{align*}
	doesn't look very promising.

	
	\subsubsection{Covariance by Ito, q=0}
	Write
	\begin{align*}
		dY(T) & = 
		\ind_{[0,t]}(T)\left(\Big( \eta- c_0 X(T) + \int f(u-T) X(u)du \Big)dT
						+ \int_{\Rm_0}c_\nu X(T-)z^2 \td N(dz,dT)\right)
		   \\
		& = dX(t\wedge T)
		   \\
		dY_h(T) & = 
		\ind_{[0,t+h]}(T)\left(\Big( \eta- c_0 X(T) + \int f(u-T) X(u)du \Big)dT
						+ \int_{\Rm_0}c_\nu X(T-)z^2 \td N(dz,dT)\right)
		   \\
		& =  dX((t+h)\wedge T)
	\end{align*}
	so that $Y(T) = X(t)$ for all $T>t$ and $Y_h(T)= X(t+h)$ for all $T>t+h$. By Ito's product formula, (Example 9.7, p.167, \cite{DiNunnoOksendalProske2009})
	\begin{align*}
		d(Y(T)Y_h(T)) = Y(T-) dY_h(T)+  Y_h(t-) dY(t) 
		+\ind_{[0,t\wedge(t+h)]}(T) \int_{\Rm_0} c_\nu^2 X(T-)^2 z^4 N(dz,dT).
	\end{align*}
	Fixing $T>t+h$, first term becomes
	\begin{align*}
		&\int_0^T Y(s-)dY_h(s)  =  \int_0^T X(t\wedge s) dY_h(s)
		   \\
		& = \int_0^{t+h} X(t\wedge s) \Big( \eta- c_0 X(s) + \int f(u-s) X(u)du \Big)ds
		+\int_0^{t+h}\int_{\Rm_0}  X(t\wedge s) \Big(c_\nu X(s-)z^2\Big) \td N(dz,ds)
		   \\
		& = \int_0^{t} X(s) \Big( \eta- c_0 X(s) + \int f(u-s) X(u)du \Big)ds
		+\int_0^{t}\int_{\Rm_0}  c_\nu X(s-)^2z^2  \td N(dz,ds)
		   \\
		& \quad+\int_t^{t+h} X(t) \Big( \eta- c_0 X(s) + \int f(u-s) X(u)du \Big)ds
		+\int_t^{t+h}\int_{\Rm_0}  X(t) \Big(c_\nu X(s-)z^2\Big) \td N(dz,ds).
	\end{align*}
	Notice here the integrands of the stochastic integrals are adapted. Second term:
	\begin{align*}
		&\int_0^T Y_h(s-)dY(s)  =  \int_0^T X((t+h)\wedge s) dY(s)
		   \\
		& = \int_0^{t} X((t+h)\wedge s) \Big( \eta- c_0 X(s) + \int f(u-s) X(u)du \Big)ds
		+\int_0^{t} \int_{\Rm_0} X((t+h)\wedge s) \Big(c_\nu X(s-)z^2\Big) \td N(dz,ds)
		   \\
		& = \int_0^{t} X(s) \Big( \eta- c_0 X(s) + \int f(u-s) X(u)du \Big)ds
		+\int_0^{t}\int_{\Rm_0}  c_\nu X(s-)^2z^2  \td N(dz,ds).
	\end{align*}
	Taking expectations:
	\begin{align*}
		&\Em(X(t+h)X(t))  =\Em(X(0)X(h))+ c_\nu^2 \kappa_4 \int_0^t \Em(X(s)^2) ds
		   \\
		& \quad+  2 \eta \int_0^t \Em(X(s)) ds - 2c_0\int_0^t \Em(X(s)^2) ds 
		+ 2 \int_0^t \int f(u-s) \Em(X(u)X(s)) du ds
		   \\
		& \quad + \eta h \Em(X(t)) - c_0\int_t^{t+h} \Em(X(t)X(s)) ds 
		+ \int_t^{t+h}\int f(u-s)\Em(X(u)X(t)) du ds.
	\end{align*}
	Recall that the mean is given by
	\begin{align*}
		m_X(t) & =  m_X(0) -c_0 \int_0^t m_X(s) ds + \int_0^t \int f(u-s)m_X(u) du ds
		   \\
		m_X(t+h) & =  m_X(0) -c_0 \int_0^{t+h} m_X(s) ds + \int_0^{t+h} \int f(u-s)m_X(u) du ds.
	\end{align*}
	By a similar product rule, 
	\begin{align*}
		&m_X(t)m_X(t+h)  = m_X(0)m_X(h)
		   \\
		& \quad + 2 \eta\int_0^t m_X(s) ds -2c_0 \int_0^t m_X^2(s) ds 
		+ 2\int_0^t \int f(u-s) m(s)m(u) du ds 
		   \\
		& \quad + \eta h m_X(t) - c_0\int_t^{t+h} m_X(s)m_X(t) ds + \int_t^{t+h}\int f(u-s) X(u)x(t) du ds.
	\end{align*}
	Therefore, denoting $C_X(t,s)=\Cov(X(t),X(s))$ and $V_X(t) = \Var(X(t))$, we have
	\begin{align*}
		C_X(t,t+h) & = C_X(0,h) 
		   \\
		& \quad+ (c_\nu^2 \kappa_4 -2c_0)\int_0^t V_X(s) ds 
		+ c_\nu^2 \kappa_4\int_0^t m_X^2(s) ds 
		+ 2\int_0^t\int f(u-s) C_X(u,s) du ds
		   \\
		& \quad -c_0\int_t^{t+h} C_X(t,s)ds + \int_t^{t+h}\int f(u-s) C_X(t,u) du ds.
	\end{align*}
	Using the formula for the variance derived earlier, we have
	\begin{align*}
		C_X(t,t+h) = C_X(0,h) + V_X(t) - V_X(0)-c_0\int_t^{t+h} C_X(t,s)ds + \int_t^{t+h}\int f(u-s) C_X(t,u) du ds.
	\end{align*}
	Changing variables,
	\begin{align*}
		&C_X(t,t+h) - C_X(0,h) - V_X(t) + V_X(0)  
			\\
		& =  -c_0\int_0^{h} C_X(t,t+s)ds + \int_0^{h}\int_{-p}^0 f(u) C_X(t,t+s+u) du ds
		   \\
		& =  \int_{-p}^0  \int_0^{h} C_X(t,t+s)ds \td\mu(du),
	\end{align*}
	where $\td\mu(du) = -c_0\delta_0(du)+ f(u) du$.
	Again, assuming second order stationarity,
	\begin{align*}
		\gamma_X(h) = \gamma_X(h) + V_X - V_X - c_0 \int_t^{t+h} \gamma_X(t-s) ds 
		+ \int_{t}^{t+h} \int _{[s-p,s]}f(u-s) \gamma_X(t-u)du ds
		\end{align*}
	which gives
	\begin{align*}
		c_0 \int_t^{t+h} \gamma_X(s-t) ds & = \int_{t}^{t+h}\int_{[s-p,s]} f(u-s) \gamma_X(u-t)du ds
		   \\
		c_0 \int_0^{h} \gamma_X(s) ds& = \int_{t}^{t+h}\int_{[-p,0]} f(u) \gamma_X(u-t+s)du ds.
	\end{align*}
	Differentiating, we have
	\begin{align*}
		c_0 \gamma_X(h) = \int_{-p}^0 f(u) \gamma_X(u+h) du
	\end{align*}
	I'm pretty sure this is incorrect - the only solution to this is the zero solution. Can't figure out where it went wrong though.
	\subsubsection{Another thought for the variance}
	First,
	\begin{align*}
		\int_{(-q,t]} F(t,s)X(s-)dS(s) & = \kappa_2 \int_{-q}^t F(t,s)X(s) ds+
		\int_{(-q,t]} F(t,s)X(s-)d\td S(s)  
		   \\
		& = \kappa_2 \int_{0}^t \int_{s-q}^s f_\nu(s-u) X(u) du ds+
		\int_{(-q,t]} F(t,s)X(s-)d\td S(s) 
	\end{align*}
	and we could write
	\begin{align*}
		X(t) & =  X(0) + \int_0^t\left(\eta - c_0 X(s) +  \int_{s-r}^s f(u-s) X(u)du\right)ds 
		+c_\nu \int_{(0,t]} X(s-)d\td S(s) + \int_{(-q,t]}F(t,s)X(s-)d\td S(s)
		   \\
		& = X(0) + \int_0^t \alpha(s) ds + \int \gamma_1(s) d\td S(s) + \int \gamma_2(s) d\td S(s) 
	\end{align*}
	Computations of $X(t)^2$:
	\begin{align*}
		X(t)^2 = X(0)X(t)+ \int_0^t X(t) \alpha(s) ds + X(t)\int \gamma_1(s) d\td S(s) 
		+ X(t)\int \gamma_2(s) d\td S(s)
	\end{align*}
	term by term: first
	\begin{align*}
		\Em(X(0)X(t))= C_X(0,t)
	\end{align*}
	second
	\begin{align*}
		\Em \left(\int_0^t X(t) \alpha(s) ds\right)
		= \eta t m_X(t) -c_0\int_0^t C_X(t,s)ds + \int_0^t \left(\int f(u-s) C_X(t,u) du\right) ds
	\end{align*}
	third
	\begin{align*}
		&c_\nu X(t)\int_0^t X(s-)d\td S(s)
		   \\
		& = c_\nu X(0)\int_0^t X(s-)d\td S(s)
		   \\
		& \quad +  c_\nu\left(\int_0^t\left(\eta - c_0 X(s) +  \int_{s-r}^s f(u-s) X(u)du\right)ds \right)\left(\int_0^t X(s-)d\td S(s)\right)
		\\&\quad+\left(c_\nu \int_{(0,t]} X(s-)d\td S(s)\right)^2
		   \\
		& \quad + c_\nu\left(\int_{(-q,t]}F(t,s)X(s-)d\td S(s)\right)\left(\int_0^t X(s-)d\td S(s)\right)
	\end{align*}
	with expectation
	\begin{align*}
		\Em \left( c_\nu X(t)\int_0^t X(s-)d\td S(s) \right)= 0 + 0 
		+ c_\nu^2 \kappa_4 \int_0^t \Em(X(s)^2) ds
		+ c_\nu \kappa_4 \int_0^t F(t,s) \Em(X(s)^2) ds.
	\end{align*}
	Last term
	\begin{align*}
		&X(t)\int_{(-q,t]}F(t,s)X(s-)d\td S(s)
		   \\
		& = X(0)\left(\int_{(-q,t]}F(t,s)X(s-)d\td S(s)\right)
		   \\
		& \quad +\left(\int_0^t\left(\eta - c_0 X(s) +  \int_{s-r}^s f(u-s) X(u)du\right)ds \right) 
				\left(\int_{(-q,t]}F(t,s)X(s-)d\td S(s)\right)
		\\&\quad+\left(c_\nu \int_{(0,t]} X(s-)d\td S(s)\right)\left(\int_{(-q,t]}F(t,s)X(s-)d\td S(s)\right)
		   \\
		& \quad + \left(\int_{(-q,t]}F(t,s)X(s-)d\td S(s)\right)^2.
	\end{align*}
	Last two terms in the expression are simple, with expectation
	\begin{align*}
		c_\nu \kappa_4 \int_0^t F(t,s)\Em(X(s)^2) ds + \kappa_4 \int_0^t F(t,s)^2 \Em(X(s)^2) ds.
	\end{align*}
	Write 
	\begin{align*}
		\int_{(-q,t]}F(t,s)X(s-)d\td S(s) = \int_0^t \int_{s-q}^s f_\nu(u-s) X(u-) d\td S(u) ds
	\end{align*}
	We still need 
	\begin{align*}
		&X(0)\left(\int_{(-q,t]}F(t,s)X(s-)d\td S(s)\right)
		\\
		&\quad+\left(\int_0^t\left(\eta - c_0 X(s) +  \int_{s-r}^s f(u-s) X(u)du\right)ds \right) 
				\left(\int_{(-q,t]}F(t,s)X(s-)d\td S(s)\right)
	\end{align*}
	still doesn't solve the problem though. No matter what I do here, can't get around the expected value of the cross termspectral decompositionis there anyway around this problem?


	\subsubsection{Process Y} 
	The price process
	\begin{align*}
		Y(t) - Y_0=  \int_{0+}^t \rt{X(s-)} dL(s), \quad t> 0
	\end{align*}
	satisfies
	\begin{align*}
		\Em [Y(t)] & =  \Em[Y_0]
		   \\
		\Var(Y(t)|Y_0)& = \td \kappa_2 \int_{0+}^t \Em[X(s-)] ds.
	\end{align*}
	Assuming $X$ is in the stationary regime, that is $\Em[X(t)] = m_X$ for all $t$, then 
	\begin{align*}
		\Var(Y(t)|Y_0)& =\Cov(Y(t+h), Y(t)|Y_0)= \td \kappa_2 m_X t.
	\end{align*}
	Fix $\tau>0$, define the return process $(Y^{(\tau)}(t))_{t> 0}$ by 
	\begin{align*}
		Y^{(\tau)}(t)= Y(t+\tau) - Y(t)  = \int_{t+}^{t+\tau} \rt{X(s-)} dL(s).
	\end{align*}
	Then $Y^{(\tau)}$ is a second order stationary process with
	\begin{align*}
		\Em [Y\d{\tau}(t)] & =  0
			\\
		\Var (Y\d{\tau}(t)) & =  \td \kappa_2\int_{t+}^{t+\tau} \Em X(s-)  ds = \td \kappa_2 \tau m_X
		   \\
		\Cov(Y\d{\tau}(t), Y\d{\tau}(t+h)) & = \ind_{\{\tau>h\}} (\tau - h) \td\kappa_2m_X.
	\end{align*}
	Assume $h>\tau$. By It\^o's lemma, 
	\begin{align*}
		 Y\d{\tau}(t)^2 
		& =  (Y(t+\tau) - Y(t))^2
		   \\
		& = 2\int_{t+}^{t+\tau} Y(s-) \rt{X(s-)} dL(s) + \int_{t+}^{t+\tau} X(s-) d[L,L](s)
		   \\
		& = 2\int_{t+}^{t+\tau} Y(s-) \rt{X(s-)} dL(s) 
			+ \td\kappa_2\int_{t+}^{t+\tau} X(s) ds
		 	+\int_{t+}^{t+\tau}\int_{\Rm_0} X(s-) z^2 \td N(dz, ds)
	\end{align*}
	Consider
	\begin{align*}
		Y^{(\tau)}(t)^4 & =  (Y(t+\tau) - Y(t))^2
		   \\
		& = \int_{t+}^{t+\tau} 4Y(s-)^3 \rt{X(s-)} dL(s) + \int_{t+}^{t+\tau}6 Y(s-)^2 X(s-) d[L,L](s)
	\end{align*}
	\begin{align*}
		(Y(t)-Y(0))^2 X(t) & =  X(t) \left(\int_{0+}^t \rt{X(s-)} dL(s)\right)^2
		   \\
		& = X(t) \left(2\int_{0+}^{t} Y(s-) \rt{X(s-)} dL(s) + \int_{0}^{t} X(s-) d[L,L](s)\right)
	\end{align*}
	Taking expectation yields
	\begin{align*}
		\Em Y\d{\tau}(t)^2  = 
	\end{align*}
	\begin{align*}
		\Em\left[Y^{(\tau)}(t)^2\ Y\d{\tau}(t+h)^2 \right] & =  \Em\left[Y^{(\tau)}(0)^2\ Y\d{\tau}(h)^2 \right]
		   \\
		& = \Em\left[(Y(\tau) - Y(0))^2 \left(
			\int_{h+}^{h+\tau} \rt{X(s-)} dL(s)\right)^2 \right]
	\end{align*}
	

	\subsubsection{Between jumps}
	Recall $\td \kappa_2 = \int_{\Rm_0} z^2 \Pi_L(dz)+ \sigma_L^2$ and $c_0  = c_\mu - \td\kappa_2 c_\nu$. Let $T_0, T_1, \cdots$ be the jump times of the subordinator $S(t) = \td \kappa_2 t + \tilde S(t)$. For each $j\in \N_0$, $X$ follows a deterministic delay equation
	\begin{align*}
		\frac{d}{dt}X(t) = \eta - c_0 X(t) + \int_{-p}^0 f(u) X(t+u) du, \quad t \in (T_j, T_{j+1}),
		\numberthis\label{eq_p0/FDEbetweenjumps}
	\end{align*}
	with initial condition ${X(u), u\in [T_j - p, T_j]}$.
	Let $\cL_X(\xi) = \int_{0}^{\infty} e^{-\xi t} X(s)dt$ be the Laplace transform of $X$. 
	The Laplace transform of a convolution product $(f*g) (t) := \int_0^t f(u) g(t-u) du$ is given by $\cL_f(\xi) \cL_f (\xi)$. Rewriting the delay integral into
	\begin{align*}
		\int_{-p}^0 f(u) X(t+u) du & = \int_{t-p}^t f(u-t) X(u) du
		   \\
		& = \int_0^t  X(u) f(-(t-u))\ind_{[0,p]}(t-u) du
		   \\
		& =  \left(X *		f(-\cdot)\ind_{[0,p]}(\cdot)  \right)(t),
	\end{align*}
	we have
	\begin{align*}
		\cL_{X *		f(-\cdot)\ind_{[0,p]}(\cdot)}(\xi)
		& = \cL_X(\xi) \cL_{f(-\cdot)\ind_{[0,p]}(\cdot)}(\xi)
		   \\
		& = \cL_X(\xi)\int_0^p e^{-\xi t} f(-t) dt
	\end{align*}
	Furthermore, by the properties of the Laplace transform, we have $\cL_{\dot X} =  \cL_X(\xi)/\xi - X(0)$ and $\cL_{\eta} = 1/\xi$. Taking Laplace transforms of both sides of \eqref{eq_p0/FDEbetweenjumps} then yields
	\begin{align*}
		\frac{1}{\xi} \cL_X(\xi) - X(0) = \frac{\eta}{\xi} - c_0 \cL_X(\xi) + \cL_X(\xi)\int_0^p e^{-\xi t} f(-t) dt, 
	\end{align*}
	which gives
	\begin{align*}
		\cL_X(\xi) = \frac{\eta + X(0)\xi  }{1 + \Big(c_0- \int_0^p e^{-\xi t} f(-t) dt\Big)\xi}.
	\end{align*}
	We can then numerically invert the Laplace transform to get the solution. 

	\subsubsection{Convoluted L\'evy Process}
	For $t\ge 0$, denote
	\begin{align*}
		J(t) = \int_{\Rm} \ind_{[t-q,t]}(u) f_\nu(u-t) X(u-) d\td S(u).
	\end{align*}
	Since the function $f$ is of bounded variation on $\Rm_+$ and $\td S$ is c\`adl\`ag and of bounded variation with probability one, $J(t)$ is c\`adl\`ag and of bounded variation and hence a semimartingale.
	For the jumps of this process, 
	for $h>0$, 
	\begin{align*}
		J(t) - J(t-h) & =  \int \ind_{(t-h, t]}(u)f_\nu(u-t)X(u-) d\td S(u)
		    - \int \ind_{(t-q-h, t-q]}(u)f_\nu(u-t+h)X(u-) d\td S(u)
		   \\
		& \quad + \int \ind_{(t-q, t-h]}(u) \Big(f_\nu(u-t) - f_\nu(u-t+h)\Big) X(u-) d\td S(u),
	\end{align*}
	where the integrand is compactly supported and locally bounded, and hence the sup of the integrand is integrable with respect to $d\td S$. Taking $h$ to zero and using Dominated Convergence Theorem,
	\begin{align*}
		\Delta J(t) = J(t) - J(t-) & = 	f_\nu(0) X(t-) \Delta \td S(t) - f_\nu(-q) X(t-q) \Delta\td S(t-q)
	\end{align*}
	\begin{proposition}
		For $t\ge 0$, the jumps of $t\mapsto J(t)$ is indistinguishable from the jumps of 
		\begin{align*}
			\hat J(t):& = f_\nu(0)\int_0^t X(u-)d\td S(u) - f_\nu(-q) \int_0^t X\left((u-q)-\right)d\td S(u-q)
			   \\
			& = f_\nu(0)\int_0^t X(u-)d\td S(u) - f_\nu(-q) \int_{-q}^{t-q} X\left(u-\right)d\td S(u)
			   \\
			& = \int_{-q}^t \Big(f_\nu(0)\ind_{(0,t]}(u) - f_\nu(-q) \ind_{(-q,t-q]}(u) \Big)X(u-)d\td S(u).
		\end{align*}
	\end{proposition}
	Furthermore, for $h>0$ we have
	\begin{align*}
		\frac{J(t) - J(t-h)}{h} & =  \int \left(\frac{\ind_{(0, t]}(u)- \ind_{(0, t-h]}(u)}{h}\right)f_\nu(u-t)X(u-) d\td S(u)
		   \\
		& \quad - \int \left(\frac{\ind_{(0, t-q]}(u)- \ind_{(0, t-q-h]}(u)}{h}\right)f_\nu(u-t+h)X(u-) d\td S(u)
		   \\
		& \quad + \int \ind_{(t-q, t-h]}(u) \left(\frac{f_\nu(u-t) - f_\nu(u-t+h)}{h}\right) X(u-) d\td S(u).
	\end{align*}
	Letting $h\to0$, formally we should have the limit
	\begin{align*}
		\frac{dJ(t)}{dt} & =  \int \delta_t(u) f_\nu(u-t) X(u-) d\td S(u) - \int \delta_{t-q}(u) f_\nu(u-t) X(u-) d\td S(u)
		   \\
		& \quad + \int_{(t-q ,t)} f'_\nu(u-t) X(u-) d\td S(u)
		   \\
		& = f_\nu(0) X(t-) d\td S(t) - f_\nu(-q) X\left((t-q)-\right) d\td S(t-q) + \int_{(t-q ,t)} f'_\nu(u-t) X(u-) d\td S(u),
	\end{align*}
	since $f_\nu$ is differentiable in $(-q,0)$. 




	The process $\td X(t) = X(t) - M_X(t)$ is also a local martingale right? Assuming it is,
	\begin{align*}
		\Em(X(t) J(t)) & =  \Em(X(t)J(t) )
		   \\
		& = \Em(\td X(t) J(t)) + \Em(M_X(t)J(t)),
	\end{align*}
	where the second term is zero since $M_X$ is deterministic.
	The jumps of $\td X$ is given by
	\begin{align*}
		\Delta \td X(t) = c_\nu X(t-) \Delta S(t),
	\end{align*}
	(needs proof as well) so we have
	\begin{align*}
		\Em(\td X(t) J(t)) & = \Em [\td X, J](t)
		   \\
		& = \Em \sum_{u\le t}\Delta \td X(u)\Delta J(u)
		   \\
		& = \sum_{u\le t} \left\{c_\nu f_\nu(0) X(u-)^2 (\Delta \td S(u) )^2 
				- c_\nu f_\nu(-q) X(u-)X(u-q) \Delta \td S(u)\td S(u-q)\right\}
				   \\
		& = c_\nu f_\nu(0) \int_0^t\int_{\Rm_0} X(t-)^2 z^4 \td N(dz,dt)
		- c_\nu f_\nu(-q) \int_0^t \int_{\Rm_0} X(u-)X(u-q) z_1 z_2 \td N()
	\end{align*}
	


==> WIP/WIP_priceprocess.tex <==
%!TEX root = ../main.tex
\renewcommand{\rt}[1]{\sqrt{#1}}



==> WIP/WIP_secondmoment.tex <==
%!TEX root = ../WIP.tex
\subsection{Second moments}
\subsubsection{CDGARCH(p,0)}
	Here we investigate the case when $q=0$, in which $X$ can be obtained as a weak limit of GARCH$(p^\Delta, 1)$ processes. Since we don't need to define $L$ for $t<0$, we will let $(L(t))_{t\ge 0}$ be a locally square integrable L\'evy process with L\'evy-Khintchine representation
	\begin{align*}
		\Em\left[e^{iuL(t)}\right]	= \exp\left(t \left(-\frac{1}{2}\sigma_L^2 u^2 
		+ \int_{\Rm_0}(e^{iuz} - 1 - iuz)\Pi_L(dz)\right)\right),
	\end{align*}
	and let $S=[L,L]$ be its quadratic variation process. Write $\td \kappa_2 = \Em[S(1)]$ so that $\td S(t) = S(t)- \td\kappa_2t$ is a locally square integrable martingale. Recall $c_0  := c_\mu- \td\kappa_2c_\nu$.   
	The CDGARCH$(p,0)$ process $(Y(t), X(t))_{t\ge -p}$ can then be specified by a pair of stochastic functional differential equations
	\begin{align*}
		dY(t) & =   \rt{X(t-)} dL(t),
		   \\
		dX(t) 
			& =   \left(\eta - c_0 X(t) + \int_{-p}^0 f_\mu(u)X(t+u)  du\right) dt 
			+ c_\nu  X(t-) d\td S(t) \numberthis\label{eq_p0/SDE} ,
	\end{align*}
	for $t> 0$, with initial conditions $Y(0)  = Y_0$ and $X(u) = X_0(u)$ on $[-p,0]$. We will in fact assume $X$ is in the mean stationary regime given by Theorem \ref{theorem_stationarymean}, i.e., the condition $c_0   > \int_{-p}^0 f_\mu(u) du$ is satisfied,  and we have picked the initial condition
	$X_0$ with $\Em X_0 \equiv m_X$, so that $\Em[X(t)] = m_X$ for all $t$. 

	\subsubsection{Variance of CDGARCH(p,0)}
	Applying It\^o's Lemma to $x\map x^2$, we have
	\begin{align*}
		dX(t)^2  & =  2X(t-) dX(t) + [X,X](t)
		   \\
		& = 2X(t) \left(\eta -  c_0 X(t) + \int_{-p}^0 f(u)X(t+u)  du\right) dt 
		+ 2 c_\nu X(t-)^2 d\td S (t)
		   \\
		& \quad
		+ c_\nu^2 X(t-) d[\td S,\td S](t),
	\end{align*}
	which gives
	\begin{align*}
		\Em\left[X(t)^2\right] & = \Em\left[X(0)^2\right] + 2 \eta \int_0^t \Em [X(s)] ds 
		+ (\kappa_4 c_\nu^2 - 2 c_0)\int_0^t \Em \left[X(s)^2\right] ds 
		   \\
		& \quad + 2\int_0^t \int_{-p}^0 f(u) \Em\left[X(s)X(s+u)\right] du ds.\numberthis\label{eq_p0/EX^2}
	\end{align*}
	Recall from \eqref{eq_firstmoment/FDE}, the mean of the process $X$ satisfies
	\begin{align*}
		\dot m^X(t) = \eta - c_0 m^X(t) + \int_{-p}^0 f(u) m^X(s+u) du.
	\end{align*}
	Using the change of variable formula, 
	\begin{align*}
		m^X(t)^2 
		& =    m^X(0)^2 + 2\int_0^t m^X(s) \dot m^X(s) ds
		   \\
		& = m^X(0)^2 + 2 \eta\int_0^t m^X(s) ds - 2c_0 \int_0^t m^X(s)^2 ds 
			\\
		&\quad+ 2\int_0^t\int_{-p}^0 f(u) m^X(s)m^X(s+u) du ds.\numberthis\label{eq_p0/mX^2}
	\end{align*}
	From here on, we will denote $V^X(t):= \Var(X(t))$ and $C^X(t):= \Cov(X(t), X(s))$. Combining \eqref{eq_p0/EX^2} and \eqref{eq_p0/mX^2}, we have
	\begin{align*}
		V^X(t)  & =   \Em(X(t)^2) - \Em(X(t))^2
		   \\
		& = 
		V_X(0) + (\kappa_4 c_\nu^2- 2c_0)\int_0^t V_X(s) ds + \kappa_4 c_\nu^2 \int_0^t m^X(s)^2 ds
		   \\
		& \quad + 2 \int_{0}^{t}\int_{-p}^0 f(u) C_X(s,s+u) du ds.\numberthis\label{eq_p0/V(t)}
	\end{align*}
	Differentiating, we have a functional differential equation for the variance
	\begin{align*}
		\frac{d}{dt} V^X(t) = \kappa_4 c_\nu^2  m_X^2  + (\kappa_4 c_\nu^2- 2c_0)V_X(t) 
		+ 2 \int_{-p}^0 f(u) C_X(t,t+u) du,\numberthis\label{eq_p0/dV(t)}
	\end{align*}
	with initial condition $\{C_X(0, u), u\in [-p,0]\}$. 
	
	\subsubsection{Covariance of CDGARCH(p,0)}
	For $t>0$ and some fixed $h>0$, we can write
	\begin{align*}
		\Em[X(t)X(t+h)] & =  \Em[X(t)^2] + \Em[X(t) (X(t+h) - X(t))].
	\end{align*}
	From \eqref{eq_p0/SDE}, the second term can be written as 
	\begin{align*}
		X(t) (X(t+h) - X(t))& =\int_{t}^{t+h}X(t) dX(s)   
			\\
		& = \int_t^{t+h} X(t)  \left( \eta - c_0 X(s) + \int_{-p}^0 f(u)X(s+u) du \right) ds
		   \\
		& \quad + c_\nu \int_t^{t+h} \int_{\Rm_0}  X(t)X(s-) z^2 \td N(dz,ds).
	\end{align*}
	Therefore,
	\begin{align*}
		\Em[X(t)X(t+h)] & =  \Em[X(t)^2] + \eta h \Em[X(t)] - c_0 \int_{t}^{t+h} \Em[X(t)X(s)] ds
		   \\
		& \quad + \int_{t}^{t+h} \int_{-p}^0 f(u) \Em[X(t) X(s+u)] du ds. \numberthis\label{eq_p0/EX(t)EX(t+h)}
	\end{align*}
	Similarly, 
	\begin{align*}
		m^X(t)m^X(t+h)  & =m^X(t)^2 + m^X(t)\left(m^X(t+h) - m^X(t)\right)
		   \\
		& =  m^X(t)^2 + \int_{t}^{t+h} m^X(t) dm^X(s)
		   \\
		& =   m^X(t)^2 + \eta h m^X(t) - c_0 \int_t^{t+h} m_X(t) m_X(s) ds 
		   \\
		& \quad +
		\int_t^{t+h} \int_{-p}^0 f(u) m^X(t)m^X(s+u)du ds.\numberthis\label{eq_p0/m(t)m(t+h)}
	\end{align*}
	Putting \eqref{eq_p0/EX(t)EX(t+h)} and \eqref{eq_p0/m(t)m(t+h)} together, we have
	\begin{align*}
		C^X(t,t+h) & =  V^X(t) -c_0 \int_t^{t+h} C^X(t,s) ds + \int_t^{t+h} \int_{-p}^0 f(u)C^X(t, s+u) du ds
		   \\
		& = V^X(t) -c_0 \int_0^{h} C^X(t,t+s) ds + \int_0^{h} \int_{-p}^0 f(u)C^X(t, t+s+u) du ds. 
		\numberthis\label{eq_p0/C(t,t+h)}
	\end{align*}
	Differentiating, we have
	\begin{align*}
		\frac{d}{dh} C^X(t,t+h) =-c_0 C^X(t,t+h) + \int_{-p}^0 f(u) C^X(t,t+h+u) du,
	\end{align*}
	and
	\begin{align*}
		\frac{d}{dt} C^X(t,t+h) =\frac{d}{dt}V^X(t) -c_0\int_0^h \frac{d}{dt} C^X(t,t+s)  ds
		 + \int_0^h\int_{-p}^0 f(u)\frac{d}{dt} C^X(t,t+s+u) du ds,
	\end{align*}
	\subsubsection{Stationary regime of CDGARCH(p,0)}
	Assuming $X$ is second order stationary, i.e. 
	\begin{align*}
		V^X(t)=V_X, \quad m^X(t) = m_X = \frac{\eta}{c_0 - \int_{-p}^0f(u)du},\qand C^X(t,s) = C_X(t-s),
	\end{align*}
	the equation \eqref{eq_p0/dV(t)} becomes
	\begin{align*}
		V_X  = \frac{1}{(2c_0-\kappa_4c_\nu^2)} 
		\left(\frac{\kappa_4 c_\nu^2 \eta^2}{\left(c_0 - \int f(u)du\right)^2} + 2\int_{-p}^0 f(u) C_X(u) du\right),
	\end{align*}
	or as a equation of the covariance,
	\begin{align*}
		\int_{-p}^0  C_X(u)f(u) du& = 
		\left(c_0-\frac{\kappa_4c_\nu^2}{2}\right)V_X -\frac{\kappa_4 c_\nu^2 \eta^2}{2\left(c_0 - \int f(u)du\right)^2},
	\end{align*}
	i.e., if we let $k_0= - (c_0 - \kappa_4 c_\nu^2/2)$ and 
	$k_1 = -\frac{\kappa_4 c_\nu^2 \eta^2}{2\left(c_0 - \int f(u)du\right)^2}$, we have
	\begin{align*}
		k_0 C(0) + \int_{-p}^0 f(u) C(u) du = k_1
	\end{align*}
	For the covariance, \eqref{eq_p0/C(t,t+h)} becomes
	\begin{align*}
		C_X(h) & =  V_X - c_0 \int_t^{t+h} C_X(s-t) ds + \int_t^{t+h} \int_{-p}^0f(u) C_X(s+u-t) du ds
		   \\
		& = C_X(0) - c_0 \int_0^{h} C_X(s) ds + \int_0^{h} \int_{-p}^0f(u) C_X(s+u) du ds.
	\end{align*}
	The process $X$ is mean square continuous so the covariance function $C_X$ is continuous.  Therefore, the stationary covariance satisfies the functional differential equation
	\begin{align*}
		\frac{d}{dh} C_X(h)  = -c_0 C_X(h) + \int_{-p}^0 f(u)C_X(h+u) du,
	\end{align*}
	with initial condition $\{C_X(u), u\in [-p,0]\}$ that satisfies
	\begin{align*}
		k_0 C(0) + \int_{-p}^0 f(u) C(u) du = k_1
	\end{align*}

	

==> WIP/WIP_simulations.tex <==
%!TEX root = ../main.tex
\newpage\subsection{Simulation of sample paths}
	We now outline a simple Euler discretization scheme to simulate the sample paths of the process $(Y(t),X(t))_{t\ge -r}$ given by \eqref{eq_CDGARCH_Y} and \eqref{eq_CDGARCH_X}. Fix $r, T>0$, we divide the interval $[0,T]$ into a uniform grid of $N+1$ points with time steps of size $\delta=1/N$. For a $\delta>0$, we construct a process $(\bar Y^{(\delta)}(t), \bar X^{(\delta)}(t))_{t\ge -r}$, which is constant between consecutive grid points, as an approximation of $(Y, X)$. 

	For easy of notation, we will write $(\bar Y, \bar X)$ for $(\bar Y^{(\delta)}, \bar X^{(\delta)})$. 
	Fix $\delta>0$, we will write $\bar U_{n} := \bar U(n \delta)$ for any process $U$ and integer $n$. Given an initial point $Y_0\in\Rm_+$ for the process $Y$, we set $\bar Y_0 = Y_0$. For each $n\ge 1$, we approximate $Y(n \delta)$ via an Euler scheme by $\bar Y_n := \bar Y_{n-1} + {\bar X_{n-1}}^{1/2} \Delta L_n$, where $\Delta L_n = L_n - L_{n-1}$ is the increment of the driving noise $L$ over the interval $((n-1)\delta, \delta]$. Given an initial condition $X_0\in\D_{[-r,0]}$, we set $\bar X_n = X_0(n \delta)$, for $-r/\delta \le n\le 0$. For $1 \le n\le T/\delta$, we approximate $X(n \delta)$ with Euler scheme by setting
	\begin{align*}
		\bar X_n  & =   \bar X_{n-1}+ \delta\left(\eta - c_\mu \bar X_{n-1}\right) + c_\nu \bar X_{n-1} \Delta S_n
		   \\
		& \quad+ \delta\left(\int_{-p}^0 f_\mu(u) \bar X(n \delta+u) du 
			+\int_{-q}^0 f_\nu(u) \bar X(n \delta+u) dS(n \delta+ u) \right),
	\end{align*}
	where $\Delta S_n:= S_n  - S_{n-1} = [L,L](n \delta) - [L,L]( (n-1)\delta)$ is the increment of the quadratic variation of the driving noise $L$. We can further approximate the moving average integrals via a Riemann sum
	\begin{align*}
		\int_{-p}^0 f_\mu(u) \bar X(n \delta+u) du 
			\approx \sum_{k=1}^{p/\delta} \delta f_\mu(-k \delta)\bar X_{n-k},
	\end{align*}
	and
	\begin{align*}
		\int_{-q}^0 f_\nu(u) \bar X(n \delta+u) dS(n \delta+ u)
			\approx \sum_{k=1}^{q/\delta} f_\nu(-k \delta)\bar X_{n-k} \Delta S_{n-k+1},
	\end{align*}
	which, upon rearrangements, gives
	\begin{align*}
		\bar X_n   \approx  \delta \eta &
		+ \sum_{k=1}^{p/\delta}  \left( \delta^2f_\mu(-k \delta)
			+ (1-c_\mu \delta)\ind_{ \{k=1\}}\right)\bar X_{n-k}
		   \\
		 \quad&+\sum_{k=1}^{q/\delta} \left(\delta f_\nu(-k \delta)+c_\nu\ind_{ \{k=1\}}\right)
		 	\bar X_{n-k} \Delta S_{n-k+1}.
	\end{align*}
	In other words, the process $(\bar Y_n, \bar X_n)_{n\ge 1}$ approximately follows a discrete time GARCH$(\frac{p}{\delta}, \frac{q}{\delta})$ process, driven by the i.i.d. noise sequence $(\Delta L_n)_{n\ge 1}$. This analogy is not exact of course, since in general we only have $\Delta S_k \approx (\Delta L_k)^2$ for small $\delta$. 

	Let $L$ be a centered L\'evy process with triplet $(0, \sigma_L^2, \Pi_L)$. We will assume that the pure jump part of $L$ is a compound Poisson process with intensity $\lambda_L$ and jump distribution $Z_i\iidsim \cN(\mu_J, \sigma_J^2)$. This gives $\td \kappa_2 := \Em [L,L](1) = \Em L(1)^2 = \lambda (\sigma_J^2+ \mu_J^2) + \sigma_L^2$ where $\td \kappa_2$ was defined in equation \eqref{eq_drivingnoise/S}.
	By stationarity of increment, $\Delta L_{n}\stackrel{\cD}{=}\left(B(\delta) - B(0)\right) + \sum_{k=1}^{N(\delta)} Z_i$, 
	where $N(\delta)$ follows a Poisson distribution with intensity $\delta \lambda_L$. Similarly, the quadratic variation can be approximated by $\Delta S_{n} \stackrel{\cD}{=} S(\delta) =\delta \sigma_L^2+  \sum_{k=1}^{N(\delta)} Z_i^2$.

	To illustrate, we have chosen exponentially decaying delay effects in the form of 
	\begin{align*}
		f_\mu(u) = w_\mu \left(e^{\lambda_\mu u} - e^{-\lambda_\mu p}\right), \qand
		f_\nu(u) = w_\nu \left(e^{\lambda_\nu u} - e^{-\lambda_\nu q}\right),
	\end{align*}
	where $w_\mu, w_\nu, \lambda_\mu, \lambda_\nu>0$, with point masses $c_\mu<0$ and $c_\nu>0$ from the expressions \eqref{eq_mu} and \eqref{eq_nu}. These choices then gives
	$\int_{-p}^0 f_\mu (u) du  = w_\mu \left( \lambda_\mu^{-1} -e^{-\lambda_\mu p}(\lambda_\mu^{-1} + p)\right)$
	and 
	$\int_{-q}^0 f_\nu (u) du  = w_\nu \left( \lambda_\nu^{-1} -e^{-\lambda_\nu q}(\lambda_\nu^{-1} + q)\right)$. 
	The parameters are chosen to satisfy Theorem \ref{theorem_stationarymean} (\ref{theorem_stationarymean/limitingmean}), i.e., 
	\begin{align*}
		\td c := c_\mu - \td\kappa_2 c_\nu - \int_{-r} \left(f_\mu(u) + \td\kappa_2 f_\nu(u)\right) du >0,
	\end{align*}
	which gives a limiting mean of $m_X = \eta/\td c$. 

	\subsubsection{Pseudo-code}
	\begin{enumerate}
		\item Pick $r,T>0$. Pick $\delta>0$, say $0.01$. Partition $[-r,0]$ and $[0,T]$. 
		\item Pick parameters $c_\mu, c_\nu, w_\mu, w_\nu, \lambda_\mu, \lambda_\nu, \td\kappa_2$ such that $\td c>0$. Set $m_X = \eta/\td c$.
		\item Noise: fix $\sigma>0$, for $n\in \{-r/\delta, \ldots, -1,0, 1,\ldots,T/\delta\}$, 
		\begin{enumerate}
			\item draw $N(\delta)\sim \rm{Poi}(\delta \lambda_L)$,  draw $N(\delta)$ iid copies of $\cN(0, \sigma_J^2)$ and store in $Z$,
			\item set $\Delta L_n = \cN (0, \sigma_L^2\delta)+ \sum_{i=1}^{N(\delta)} Z_i$,
			\item set $\Delta S_n = \sigma_L^2 \delta + \sum_{i=1}^{N(\delta)} Z_i^2$.     
		\end{enumerate}
		
		\item Initialize: set $X_0\equiv m_X$ on $[-r,0]$, 
		or, $\bar X_n = m_X$ on $\{-r/\delta, \ldots, -1,0\}$. 
		Set $\bar Y_0 = Y_0$. 
		
			
		\item Recursion: for each $n\in \{1,2, \ldots, T/\delta\}$, compute $(\bar Y_n, \bar X_{n})$ by:
		\begin{enumerate}
			\item Set
			\begin{align*}
				\bar X_n   \approx  \delta \eta &
				+ \sum_{k=1}^{p/\delta}  \left( \delta^2f_\mu(-k \delta)
				+ (1-c_0 \delta)\ind_{ \{k=1\}}\right)\bar X_{n-k}
		   		\\
		 		\quad&+\sum_{k=1}^{q/\delta} \left(\delta f_\nu(-k \delta)+c_\nu\ind_{ \{k=1\}}\right)
		 		\bar X_{n-k} \Delta S_{n-k+1}.
			\end{align*}
			
			\item Set $Y_{n} = \sqrt{X_{n-1}} \Delta L_{n}$.
			
		\end{enumerate}\end{enumerate}




==> WIP/WIP_stationarity.tex <==
%!TEX root = ../main.tex
\subsection{Uniform integrability}
Proof is adapted from one of the \citeauthor{BaoYinYuanEtAl2014} papers.
Consider a CDGARCH$(p,0)$ variance process given by
\begin{align*}
	dX(t) = \left(\eta - c_0 X(t) + \int_{-p}^0 X(t+u) f(u) du\right) dt + c_\nu X(t-) d\td S(t),
	\numberthis\label{eq_p0/X}
\end{align*}
$t\ge  0$, with initial condition $X_0\in \D_{[-p,0]}$. Recall $\kappa_4:= \int_{\Rm_+} z^4 \Pi_L(dz)$. 
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}[\citet{ItoNisio1943}]\label{lem:ItoNisio}
	Suppose $u,v:[0, \infty)\to \Rm_+$ are continuous functions, $\alpha>0$ and $\lambda_1>\lambda_2>0$. For every $0\le t<\infty$, 
	\begin{enumerate}[(i).]
	\item \label{lem:ItoNisio/1} if $u(t)\le  u(0) - \lambda_1\int_{0}^t u(r) dr + \int_0^t v(r) dr$, 
		then
		\begin{align*}
			u(t)\le u(0) + \int_0^t e^{-\lambda_1(t-r)} v(r) dr.
		\end{align*}
	\item \label{lem:ItoNisio/2} if  $u(t)\le  \alpha + \lambda_2\int_{0}^t e^{-\lambda_1 (t-s)}u(r) dr$, then $u(t) \le \frac{ \lambda_1\alpha}{\lambda_1 - \lambda_2}$.
	\end{enumerate}
\end{lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proposition}
	Suppose $X(t)$ has finite $k+\epsilon$ moment for some $k\ge 1$ and $\epsilon>0$, for all $t\ge 0$. 
	If the parameters in \eqref{eq_p0/X} satisfy
	\begin{align*}
		c_0  > \norm{f}_{L^1} + \frac{k-1}{2} \kappa_4 c_\nu^2 ,\numberthis\label{eq_UI/condition}
	\end{align*}
	then there exists some small $\epsilon>0$ such that
	\begin{align*}
	 	\sup_{t\ge -r} \Em[X(t)^{k+\epsilon}]<\infty
	\end{align*} 
	In particular, $X$ is uniformly integrable if $c_0  > \norm{f}_{L^1}$.
	%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\begin{proof}
	Fix $\epsilon>0, k\ge 1$, by Ito's Lemma applied to $x\mapsto x^{k+ \epsilon}$, 
	\begin{align*}
		dX(t)^{k+ \epsilon} = (k+ \epsilon) X(t)^{k-1+\epsilon} dX(t)
		+ \frac{(k+\epsilon)(k-1+\epsilon)}{2}X(t)^{k-2 + \epsilon}d[X,X](t),
	\end{align*}
	where recall $dX(t)=(\eta - c_0 X(t) + \int_{-p}^0 f(u) X(t+u) du)dt + c_\nu X(t-) d\td S(t)$ and $d[X,X](t) = c_\nu ^2 X(t-)^2 d[\td S,\td S](t)$. 
	Writing $E(t) := \Em\left[X(t)^{k+\epsilon}\right]$, taking expectations, we have
	\begin{align*}
		E(t)  =E(0)
		+& (k+\epsilon) \Em\left[\int_0^t X(s)^{k-1+\epsilon} 
		\left(\eta - c_0 X(s) + \int_{-p}^0 f(u)X(s+u) du\right)ds \right]
		   \\
		+&\frac{(k+\epsilon)(k-1+\epsilon)}{2}
		\kappa_4 c_\nu ^2 \Em\left[\int_{-p}^0 X(s)^{k-2 +\epsilon} X(s)^2 ds\right],
	\end{align*}
	which after rearranging becomes
	\begin{align*}
		E(t)&= E(0) 
		+(k+\epsilon)\Em\left[ \int_0^t X(s)^{k-1+\epsilon}
		 \left( \eta+ \left( \frac{k-1}{2} \kappa_4 c_\nu ^2 - c_0\right) X(s) \right) ds\right]
		   \\
		& \qquad  + (k+\epsilon)\Em\left[
		\int_0^t X(s)^{k-1+\epsilon} \left(\int_{-p}^0 f(u)X(s+u) du \right)  
		+\epsilon\frac{ \kappa_4 c_\nu^2}{2} X(s)^{k+\epsilon}ds \right].
	\end{align*}
	For the first integral, observe that by assumption \eqref{eq_UI/condition} we can write
	\begin{align*}
		\frac{1}{2}\left( - c_0+\frac{k-1}{2}\kappa_4 c_\nu^2 + \norm{f}_{L^1}\right)< 0,
	\end{align*}
	which implies that there exists $c\in\Rm$ such that
	\begin{align*}
		X(s)^{k-1+\epsilon}\left(\eta + \frac{1}{2}\left(-c_0+\frac{k-1}{2}\kappa_4 c_\nu^2 + \norm{f}_{L^1}\right) X(s) \right) < c,
	\end{align*}
	for any values of $X(s)\ge 0$.  Rearranging gives
	\begin{align*}
		&X(s)^{k-1+\epsilon}
		\left(\eta+ \left( - c_0 + \frac{k-1}{2} \kappa_4 c_\nu ^2 \right) X(s) \right)
		\\
		&\qquad\qquad< c - \frac{1}{2}\left(c_0 - \frac{k-1}{2} \kappa_4 c_\nu^2 + \norm{f}_{L^1}\right) X(s)^{k+\epsilon}.
		\numberthis\label{eq_UI/bound_on_eta_term}
	\end{align*}
	For second integral, recall Young's inequality $xy\le \frac{1}{p}x^{p} + \frac{1}{q} y^{q}$,  for all  $x,y,p,q>0$  with $\frac{1}{p}+\frac{1}{q}=1$. Writing $\bar E(s) = \sup_{u\in[-p,s]} E(u)$, by Fubini's theorem, 
	\begin{align*}
		&\Em \left[X(s)^{k-1+\epsilon} \int_{-p}^0 f(u) X(s+u) ds\right]
		=\int_{-p}^0 f(u) \Em \left[X(s)^{k-1+\epsilon} X(s+u)\right] ds
		   \\
		& \qquad
		\le \norm{f}_{L^1}\sup_{u\in[-p,0]} \Em \left[ X(s)^{k-1+\epsilon}  X(s+u)\right]
		   \\
		&\qquad \le \norm{f}_{L^1}\sup_{u\in[-p,0]} \Em\left[ \frac{k-1+\epsilon}{k+\epsilon} X(s)^{k+\epsilon}  
		+\frac{1}{k+\epsilon}X(s+u)^{k+\epsilon} \right]
		   \\
		& \qquad\le \norm{f}_{L^1}\left( \frac{k-1+\epsilon}{k+\epsilon} E(s)
		+\frac{1}{k+\epsilon}\bar E(s) \right).
		\numberthis\label{eq_UI/bound_on_delay_integral}
	\end{align*}
	Combining \eqref{eq_UI/bound_on_eta_term} and \eqref{eq_UI/bound_on_delay_integral}, $E(t)$ can be bounded by
	\begin{align*}
		E(t)&\le E(0)
		- \lambda_1
		\int_0^t E(s) ds
		 +  \int_0^t\left( c'+ \lambda_2\bar E(s)\right) ds.
	\end{align*}
	where $ c' = (k+\epsilon)c$,  $\lambda_2 = \norm{f}_{L^1}$,
	\begin{align*}
		\lambda_1:& =  {(k+\epsilon)}\left(
		\frac{1}{2}\left(c_0  - \frac{k-1}{2}\kappa_4 c_\nu^2 + \norm{f}_{L^1}\right)
		- \frac{k-1+\epsilon}{k+\epsilon}\norm{f}_{L^1}
		- \frac{\epsilon}{2}\kappa_4 c_\nu^2\right),
	\end{align*}
	so that
	\begin{align*}
		\lambda_1 - \lambda_2 & = 
		{(k+\epsilon)}\left(
		\frac{1}{2}\left(c_0  - \frac{k-1}{2}\kappa_4 c_\nu^2 + \norm{f}_{L^1}\right)
		- \norm{f}_{L^1}
		- \frac{\epsilon}{2}\kappa_4 c_\nu^2\right)
		   \\
		& = {(k+\epsilon)}\left(
		\frac{1}{2}\left(c_0  - \frac{k-1}{2}\kappa_4 c_\nu^2 - \norm{f}_{L^1}\right)
		- \cO (\epsilon)\right).
	\end{align*}
	Since we have assumed $c_0- \frac{k-1}{2}\kappa_4 c_\nu^2- \norm{f}_{L^1} >0$, there exists a small enough $\epsilon>0$ such that $\lambda_1> \lambda_2 >0$. 
	By Lemma \ref{lem:ItoNisio} (\ref{lem:ItoNisio/1}), 
	\begin{align*}
		E(t)\le  E(0) + \int_0^t e^{-\lambda_1(t-s)}  \left(c'+\lambda_2\bar E(s)\right) ds. 
		\numberthis\label{eq_uniform_int_E_e}
	\end{align*}
	Since $\bar E$ is non-decreasing, a quick integration by parts shows that the integral in \eqref{eq_uniform_int_E_e} is non-decreasing with respect to $t$. Hence 
	\begin{align*}
		\bar E(t) = \sup_{u\in [-p,t]} E(u) 
		& \le E(0) + \sup_{u\in [-p,t]} \int_0^u e^{-\lambda_1(u-s)}\left(c'+\lambda_2\bar E(s)\right) ds
		   \\
		& \le E(0) + \int_0^t e^{-\lambda_1(t-s)} \left(c'+\lambda_2\bar E(s)\right) ds
		   \\
		& \le c'' + \lambda_2 \int_0^t e^{-\lambda_1(t-s)} \lambda_2\bar E(s),
	\end{align*}
	where $c'':= \Em[X(0)^{k+\epsilon}] + c'\int_0^t e^{-\lambda_1(t-s)}ds<\infty$. 
	By Lemma \ref{lem:ItoNisio} (\ref{lem:ItoNisio/2}), 
	\begin{align*}
		\sup_{u\in[-p,t]} \Em[X(u)^{k+\epsilon}] = \bar E(t) & 
		\le \frac{\lambda_1 c''}{\lambda_1 - \lambda_2} <\infty,
	\end{align*}
	since $\lambda_1>\lambda_2>0$. 
	
	\end{proof}
\end{proposition}


\subsubsection{bounds for pq}
Square ntegrability: Cauchy Schwartz, 
\begin{align*}
	\Em\left[X(t) \int_{t-q+}^t f(u-t)X(u-)d\td S(u)\right]
	&\le \Em\left[X(t)^2\right]^{1/2} 
		\Em\left[\left(\int_{t-q+}^t f(u-t)X(u-)d\td S(u)\right)^2\right]^{1/2}
		\\
	&\le \Em\left[X(t)^{2}\right]^{\frac{1}{2}} 
	\left(\int_{t-q+}^t f(u-t)^2\Em\left[X(u-)^2\right]\td\kappa_4 du\right)^{1/2}
	   \\
	&\le \td \kappa_4^{1/2}\norm{f}_{L^2} \sup_{u\le t}\Em[X(u)^2]
\end{align*}
Square uniform integrability: H\"older's inequality with $\frac{1}{p} = \frac{1+\epsilon}{2+\epsilon},\qand \frac{1}{q}= \frac{1}{2+\epsilon}$ gives
\begin{align*}
	\Em\left[X(t)^{1+\epsilon} \int_{t-q+}^t f(u-t)X(u-)d\td S(u)\right]
	&\le \Em\left[X(t)^{2+\epsilon}\right]^{1/p} 
	\Em\left[\left(\int_{t-q+}^t f(u-t)X(u-)d\td S(u)\right)^{2+\epsilon}\right]^{1/q}.
\end{align*}
Claim is that this is less than
\begin{align*}
	const.\sup_{s\le t} \Em\left[X(s)^{2+\epsilon}\right],
\end{align*}
I just don't see how. Another try with $\frac{1}{q} = \frac{1}{2}$ gives
\begin{align*}
	\Em\left[X(t)^{1+\epsilon} \int_{t-q+}^t f(u-t)X(u-)d\td S(u)\right]
	&\le \Em\left[X(t)^{2+2\epsilon}\right]^{1/2} 
	\Em\left[\left(\int_{t-q+}^t f(u-t)X(u-)d\td S(u)\right)^{2}\right]^{1/2}.
	   \\
	& \le \Em\left[X(t)^{2+2\epsilon}\right]^{1/2} 
	\left(\int_{t-q+}^t f(u-t)^2 \Em\left[X(u-)^2\right]\td \kappa_4 du\right)^{1/2}
	   \\
	& \le \td\kappa_4^{1/2} \norm{f}_{L^2}\sup_{u\le t}\Em\left[X(u)^{2+2\epsilon}\right],
\end{align*}
gives what we want, but obviously does not generalise. 


\subsubsection{}
For more general case: H\"older's inequality, 
\begin{align*}
	&\Em\left[X(t)^{\kappa-1+\epsilon} \int_{t-q+}^t f(u-t)X(u-)d\td S(u)\right]
	\le \Em\left[\left(X(t)^{\kappa-1+\epsilon}\right)^p\right]^{1/p} 
	\Em\left[\left(\int_{t-q+}^t f(u-t)X(u-)d\td S(u)\right)^q\right]^{1/q}
\end{align*}
with
\begin{align*}
	\frac{1}{p} = \frac{\kappa-1+\epsilon}{\kappa+\epsilon},\qand \frac{1}{q}= \frac{1}{\kappa+\epsilon}
\end{align*}
gives
\begin{align*}
	\Em\left[X(t)^{\kappa-1+\epsilon} \int_{t-q+}^t f(u-t)X(u-)d\td S(u)\right]
	&\le \Em\left[X(t)^{\kappa+\epsilon}\right]^{1/p} 
	\Em\left[\left(\int_{t-q+}^t f(u-t)X(u-)d\td S(u)\right)^{\kappa+\epsilon}\right]^{1/q}
\end{align*}
Burkholder's inequality gives
\begin{align*}
	&\le \Em\left[X(t)^{\kappa+\epsilon}\right]^{1/p} 
	\Em\left[\left[\int f(u-\cdot)X(u-)d\td S(u),\int f(u-\cdot)X(u-)d\td S(u)\right]_t^{\frac{\kappa+\epsilon}{2}}\right]^{1/q}
	   \\
	&\le \Em\left[X(t)^{\kappa+\epsilon}\right]^{1/p} 
	\Em\left[\left(\int f^2 X^2 d[\td S, \td S]\right)^{\frac{\kappa+\epsilon}{2}}\right]^{1/q}
\end{align*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Recall definitions of $c_0, f, \td \kappa_2$ and $\td S$ from Section \ref{section_results/pq/firstmoment}. We will rewrite the SFDE \eqref{eq_results/semimartingaleSDE} as
\begin{align*}
	dX(t) & =  \Big(\eta - c_0 X(t)\Big) dt +   c_\nu X(t-) d\td S(t) \numberthis\label{eq_results/stationarity/XwithtdS}
	   \\
	&  \qquad + \left(\int_{t-r}^t f(u-t) X(u) du + \int_{t-q+}^t f_\nu(u-t)X(u-) d\td S(u)\right)dt. 
\end{align*}

\begin{proof}[Proof of Theorem \ref{theorem_stationarity/UI}]
	Fix $\epsilon>0$. By Ito's Lemma (see \cite{DiNunnoOksendalProske2009}) applied to $x\mapsto x^{2+ \epsilon}$, 
	\begin{align*}
		dX(t)^{2+ \epsilon} = (2+ \epsilon) X(t)^{1+\epsilon} dX(t)
		+ \frac{(2+\epsilon)(1+\epsilon)}{2}X(t)^{\epsilon}d[X,X](t),
	\end{align*}
	where from \eqref{eq_results/stationarity/XwithtdS},  $d[X,X](t) = c_\nu^2 X(t-) d[\td S, \td S](t)$. 
	Writing $E(t) := \Em\left[X(t)^{2+\epsilon}\right]$, we have
	\begin{align*}
		E(t)  =E(0)
		+& (2+\epsilon) \Em\left[\int_0^t X(s)^{1+\epsilon} 
		\left(\eta - c_0 X(s)  \right)ds \right]
		   \\
		+& (2+\epsilon) \Em\left[\int_0^t X(s)^{1+\epsilon} 
		\left( \int_{s-r}^s f(u-s)X(u) du + \int_{s-q+}^s f_\nu(u)X(u-) dS(u)  \right)ds \right]
		   \\
		+&\frac{(2+\epsilon)(1+\epsilon)}{2}
		\kappa_4 c_\nu ^2 \Em\left[\int_{0}^t X(s)^{\epsilon} X(s)^2 ds\right],
	\end{align*}
	which after rearranging becomes
	\begin{align*}
		E(t)= E(0) 
		&+(2+\epsilon)\Em\left[ \int_0^t X(s)^{1+\epsilon}
		 \left( \eta+ \left( \frac{1}{2} \kappa_4 c_\nu ^2 - c_0\right) X(s) \right) ds\right]
	\\
		&   + (2+\epsilon) \Em\left[\int_0^t X(s)^{1+\epsilon} 
		\left( \int_{s-r}^s f(u-s)X(u) du + \int_{s-q+}^s f_\nu(u)X(u-) dS(u)  \right)ds \right]
	\\
		&   + \frac{(2+\epsilon)\epsilon}{2}{ \kappa_4 c_\nu^2}\Em\left[\int_{0}^t
		 X(s)^{2+\epsilon}ds \right].
		\numberthis\label{eq_proof/UI/E(t)}
	\end{align*}
	For the first integral in \eqref{eq_proof/UI/E(t)}, we first observe that by assumption \eqref{eq_results/stationarity/UIcondition} we have
	\begin{align*}
		\frac{1}{2}\left( - c_0+\frac{1}{2}\kappa_4 c_\nu^2 + \norm{f}_{L^1}\right)< 0,
	\end{align*}
	which implies that there exists $c\in\Rm$ such that for all $X(s)\ge 0$, 
	\begin{align*}
		X(s)^{1+\epsilon}\left(\eta + \frac{1}{2}\left(-c_0+\frac{1}{2}\kappa_4 c_\nu^2 + \norm{f}_{L^1}\right) X(s) \right) < c.
	\end{align*}
	Rearranging, we have a bound for the integrand:
	\begin{align*}
		&X(s)^{1+\epsilon}
		\left(\eta+ \left( - c_0 + \frac{1}{2} \kappa_4 c_\nu ^2 \right) X(s) \right)
		< c - \frac{1}{2}\left(c_0 - \frac{1}{2} \kappa_4 c_\nu^2 + \norm{f}_{L^1}\right) X(s)^{k+\epsilon}.
		\numberthis\label{eq_proof/UI/bound_on_eta_term}
	\end{align*}
	For the first term in the second integral in \eqref{eq_proof/UI/E(t)}, recall Young's inequality $xy\le \frac{1}{p}x^{p} + \frac{1}{q} y^{q}$,  for all  $x,y,p,q>0$  with $\frac{1}{p}+\frac{1}{q}=1$. Writing $\bar E(s) = \sup_{u\in[-p,s]} E(u)$, by Fubini's theorem, 
	\begin{align*}
		&\Em \left[X(s)^{1+\epsilon} \int_{-r}^0 f(u) X(s+u) du\right]
		=\int_{-r}^0 f(u) \Em \left[X(s)^{1+\epsilon} X(s+u)\right] du
		   \\
		& \qquad
		\le \norm{f}_{L^1}\sup_{u\in[-r,0]} \Em \left[ X(s)^{1+\epsilon}  X(s+u)\right]
		   \\
		&\qquad \le \norm{f}_{L^1}\sup_{u\in[-r,0]} \Em\left[ \frac{1+\epsilon}{k+\epsilon} X(s)^{k+\epsilon}  
		+\frac{1}{k+\epsilon}X(s+u)^{k+\epsilon} \right]
		   \\
		& \qquad\le \norm{f}_{L^1}\left( \frac{1+\epsilon}{k+\epsilon} E(s)
		+\frac{1}{k+\epsilon}\bar E(s) \right).
		\numberthis\label{eq_proof/UI/bound_on_delay_integral}
	\end{align*}
	Combining \eqref{eq_proof/UI/bound_on_eta_term} and \eqref{eq_proof/UI/bound_on_delay_integral}, $E(t)$ can be bounded by
	\begin{align*}
		E(t)&\le E(0)
		- \lambda_1
		\int_0^t E(s) ds
		 +  \int_0^t\left( c'+ \lambda_2\bar E(s)\right) ds.
	\end{align*}
	where $ c' = (k+\epsilon)c$,  $\lambda_2 = \norm{f}_{L^1}$, and
	\begin{align*}
		\lambda_1:& =  {(k+\epsilon)}\left(
		\frac{1}{2}\left(c_0  - \frac{1}{2}\kappa_4 c_\nu^2 + \norm{f}_{L^1}\right)
		- \frac{1+\epsilon}{k+\epsilon}\norm{f}_{L^1}
		- \frac{\epsilon}{2}\kappa_4 c_\nu^2\right),
	\end{align*}
	so that
	\begin{align*}
		\lambda_1 - \lambda_2 & = 
		{(k+\epsilon)}\left(
		\frac{1}{2}\left(c_0  - \frac{1}{2}\kappa_4 c_\nu^2 + \norm{f}_{L^1}\right)
		- \norm{f}_{L^1}
		- \frac{\epsilon}{2}\kappa_4 c_\nu^2\right)
		   \\
		& = {(k+\epsilon)}\left(
		\frac{1}{2}\left(c_0  - \frac{1}{2}\kappa_4 c_\nu^2 - \norm{f}_{L^1}\right)
		- \cO (\epsilon)\right).
	\end{align*}
	Since we have assumed $c_0- \frac{1}{2}\kappa_4 c_\nu^2- \norm{f}_{L^1} >0$, there exists a small enough $\epsilon>0$ such that $\lambda_1> \lambda_2 >0$. 
	By Lemma \ref{lem_stationarity/ItoNisio} (\ref{lem_stationarity/ItoNisio/1}), 
	\begin{align*}
		E(t)\le  E(0) + \int_0^t e^{-\lambda_1(t-s)}  \left(c'+\lambda_2\bar E(s)\right) ds. 
		\numberthis\label{eq_proof/UI/E(t)afterfirstGronwall}
	\end{align*}
	Since $\bar E$ is non-decreasing, a quick integration by parts shows that the integral in \eqref{eq_proof/UI/E(t)afterfirstGronwall} is non-decreasing with respect to $t$. Hence 
	\begin{align*}
		\bar E(t) = \sup_{u\in [-p,t]} E(u) 
		& \le E(0) + \sup_{u\in [-p,t]} \int_0^u e^{-\lambda_1(u-s)}\left(c'+\lambda_2\bar E(s)\right) ds
		   \\
		& \le E(0) + \int_0^t e^{-\lambda_1(t-s)} \left(c'+\lambda_2\bar E(s)\right) ds
		   \\
		& \le c'' + \lambda_2 \int_0^t e^{-\lambda_1(t-s)} \lambda_2\bar E(s),
	\end{align*}
	where $c'':= \Em[X(0)^{k+\epsilon}] + c'\int_0^t e^{-\lambda_1(t-s)}ds<\infty$. 
	By Lemma \ref{lem_stationarity/ItoNisio} (\ref{lem_stationarity/ItoNisio/2}), since $\lambda_1>\lambda_2>0$,
	\begin{align*}
		\sup_{u\in[-p,t]} \Em[X(u)^{k+\epsilon}] = \bar E(t) & 
		\le \frac{\lambda_1 c''}{\lambda_1 - \lambda_2} <\infty.
	\end{align*}
\end{proof}





==> numerics/numerics.tex <==
%!TEX root = ../main.tex
\section{Numerical simulation}\label{section/1/discretization}
We now outline a simple Euler scheme for the process $(Y(t),X(t))_{t\ge -r}$ given by \eqref{equation/1/model/CDGARCH_Y} and \eqref{equation/1/model/CDGARCH_X}. Fix $r, T>0$, we divide the interval $[0,T]$ into a uniform grid of $N+1$ points with time steps of size $\delta=1/N$. Fix $\delta>0$,, we construct a process $( Y^{(\delta)}_t, X_t^{(\delta)})_{t\ge -r}$, which is constant between consecutive grid points, as an approximation of $(Y, X)$. 

	For easy of notation, we will write $\bar U_{n} := U_{n \delta}^{(\delta)}$ for any process $U$ and integer $n$. 
	Given a L\'evy process $(L_t)_{t\ge -r}$, 
	let $\Delta \bar L_n = \bar L_n - \bar L_{n-1}$ be the increment of the driving noise $L$ over the interval $((n-1)\delta, \delta]$, and $\Delta \bar S_n:= \bar S_n  - \bar S_{n-1} = [L,L]_{n \delta} - [L,L]_{(n-1) \delta}$ be the increment of the quadratic variation of the driving noise $L$.
	Given an initial condition $\Phi\in\D_{[-r,0]}$, we set $\bar X_n = \Phi_{n \delta}$, for $-r/\delta \le n\le 0$.
	For $1 \le n\le T/\delta$, set
	\begin{align*}
		\bar X_n  & =   \bar X_{n-1}+ \delta\left(\eta - c_\mu \bar X_{n-1}\right) + c_\nu \bar X_{n-1}\Delta \bar S_n
		   \\
		& \quad+ \delta\left(\sum_{k=1}^{p/\delta} \delta f_\mu(-k \delta)\bar X_{n-k}
			+\sum_{k=1}^{q/\delta} f_\nu(-k \delta)\bar X_{n-k} \Delta \bar S_{n-k+1} \right),
		\\
	\end{align*}
	which becomes
	\begin{align*}
	\bar X_n = \delta \eta 
		&+\sum_{k=1}^{p/\delta}  \left( \delta^2f_\mu(-k \delta)
			+ (1-c_\mu \delta)\ind_{ \{k=1\}}\right)\bar X_{n-k}
	\\
		&+\sum_{k=1}^{q/\delta} \left(\delta f_\nu(-k \delta)+c_\nu\ind_{ \{k=1\}}\right)
		 	\bar X_{n-k} \Delta S_{n-k+1}.
	\end{align*}
	Given an initial point $Y_0\in\Rm_+$ for the process $Y$, we set $\bar Y_0 = Y_0$. For each $n\ge 1$, set $\bar Y_n := \bar Y_{n-1} + {\bar X_{n-1}}^{1/2} \Delta L_n$, 



	\begin{remark}
		In the case $q=0$, the process $(\bar Y_n, \bar X_n)_{n\ge 1}$ is a discrete time GARCH$(\lceil{p}/{\delta}\rceil, 1)$ process, driven by the i.i.d. noise sequence $(\Delta \bar L_n)_{n\ge 1}$. \cite{Tran2013} gives the weak convergence of this scheme. In the general where $q\ne0$, the discretized process $(\bar Y_n, \bar X_n)$ is no longer a GARCH process, but higher resemble one since $\Delta \bar S_k \approx (\Delta \bar L_k)^2$ for small $\delta$.
	\end{remark}

	To illustrate, we will assume that the pure jump part of $L$ is a compound Poisson process with intensity $\lambda_L$ and jump distribution $Z_i\iidsim \cN(\mu_J, \sigma_J^2)$. We have chosen exponentially decaying delay effects in the form of 
	\begin{align*}
		f_\mu(u) = w_\mu \left(e^{\lambda_\mu u} - e^{-\lambda_\mu p}\right), \qand
		f_\nu(u) = w_\nu \left(e^{\lambda_\nu u} - e^{-\lambda_\nu q}\right),
	\end{align*}
	where $w_\mu, w_\nu, \lambda_\mu, \lambda_\nu>0$, with point masses $c_\mu<0$ and $c_\nu>0$ from the expressions \eqref{equation/1/model/mu} and \eqref{equation/1/model/nu}. The parameters are chosen to give a covariance stationary $X$. {\color{red} TALKABOUT FIGURE, SHOW ACF PERHAPS. CONCLUSION} 

	\begin{figure}[H]
		\centering\includegraphics[width =12cm]{figs/example.jpg}
	\end{figure}

	



==> proofs/proofs_momentboundGENERAL_K.tex <==
%!TEX root = ../main.tex
\subsection{Moment bounds}\label{section/proofs/1/moments}
We precede the proof of Theorem \ref{theorem/1/moments/moment bound} with the following two lemmas.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55
\begin{lemma}[\citet{ItoNisio1943}]\label{lemma/1/stationarity/ItoNisio}
	Suppose $x,y:[0, \infty)\to \Rm_+$ are continuous functions, $\alpha>0$ and $\lambda_1>\lambda_2>0$. For every $0\le t<\infty$, 
	\begin{enumerate}[(i).]
	\item \label{lemma/1/stationarity/ItoNisio/1} If $x_t\le  x_0 - \lambda_1\int_{0}^t x_u du + \int_0^t y_u du$, then $x_t\le x_0 + \int_0^t e^{-\lambda_1(t-u)} y_u du.$

	\item \label{lemma/1/stationarity/ItoNisio/2} If  $x_t\le  \alpha + \lambda_2\int_{0}^t e^{-\lambda_1 (t-s)}x_u du$, then $x_t \le \alpha\lambda_1/({\lambda_1 - \lambda_2})$.
	\end{enumerate}
\end{lemma}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lemma/1/stationarity/cross}
	Suppose Assumptions \ref{assumptions/1/existence} hold and $(X_t)_{t\ge 0}$ is the (positive) unique strong solution to \eqref{equation/1/semimartingale/XSDDE} with initial condition $\Phi$. 
	Let $k\ge 1$, then
	\begin{align*}
		\Em\left[X_t^{k-1}\int_{t-p}^t f_\mu(u-t)X_u du \right]
		\le \norm{f_\mu}_{L^1} \sup_{u\in[t-r,t]}\Em[X_u ^k], \quad t> 0.
	\end{align*}
	Suppose further $S$ has finite $k$-th moment. Then there exists a constant $C_k := C_{k,\td S,f,t}$ such that
	\begin{align*}
		\Em \left[X_t^{k-1} \int_{t-q+}^t f_\nu(u-t) X_{u-} dS_u\right]
		\le C_k \norm{f_\nu}_{L^k} \sup_{u\in(t-q,t]}\Em[X_u ^k], \quad t> 0.
	\end{align*}
	In the case where $k=1,2$,  we can choose $C_1=\kappa_2$ and $C_2 = \kappa_4$.

	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\begin{proof}
	Since $X$ is positive and c\`adl\`ag, by Fubini's theorem and H\"older's inequality,
	\begin{align*}
		&\Em\left[X_t^{k-1}\int f_\mu(u-t)X_u du \right]
		= \int f_\mu(u-t)\Em[X_t^{k-1}X_u  ]du
		\\
		&\hspace{20mm}
		\le \int f_\mu(u-t)\Em[X_t^{k}]^{\frac{k-1}{k}} \Em [X_u^k]^{\frac{1}{k}}du
		\le \norm{f_\mu}_{L^1} \sup_{u\in[t-r,t]}\Em[X_u ^k].
	\end{align*}
	% For the second claim, recall $dS_t = \kappa_2 dt + d\td S_t$, we have
	% \begin{align*}
	% 	\Em \left[X_t^{k-1} \int f_\nu(u-t) X_{u-} dS_u\right]
	% 	= \kappa_2 \Em\left[X_t^{k-1} \int f_\nu(u-t) X_{u} du\right]
	% 	+\Em\left[X_t^{k-1} \int f_\nu(u-t) X_{u-} d\td S_u\right].
	% \end{align*}
	For the second claim, H\"older's inequality and Theorem V.66 of \cite{Protter2004} gives
	\begin{align*}
		&\Em \left[X_t^{k-1} \int_{t-q+}^t f_\nu(u-t) X_{u-} dS_u\right]
		\le \Em [X_t^k]^{\frac{k-1}{k}}
		\Em\left[\left(\int_{t-q+}^t f_\nu(u-t) X_{u-} dS_u\right)^k \right]^{\frac{1}{k}}
		\\
		&\hspace{2cm} \le \Em [X_t^k]^{\frac{k-1}{k}}
		{C_k} \left(\int_{t-q+}^t f_\nu(u-t)^k \Em[X_u ^k] du\right)^{\frac{1}{k}}
		\le C_k \norm{f_\nu}_{L^k} \sup_{u\in(t-q,t]}\Em[X_u^k],
	\end{align*}
	for some $C_k$ which depends on $S, f$ and $t$. For the case $k=2$, simply observe that
	\begin{align*}
		\Em\left[\left(\int_{t-q+}^t f_\nu(u-t) X_{u-} dS_u\right)^2 \right]
		= \kappa_4  \int_{t-q}^t f_\nu(u-t)^2 \Em\left[X_u ^2\right] du
	\end{align*}
	so we could choose $C_2= \kappa_4$. The $k=1$ case is trivial. 
	\end{proof}
\end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}[Proof of Theorem \ref{theorem/1/moments/moment bound}]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\pf{(\ref{theorem/1/moments/moment bound/Lk}).}
		Fix $k\ge 1$, Ito's Lemma (\cite[Theorem I.4.57]{JacodShiryaev2013}) gives, 
		\begin{align*}
			X_t^{k} =X_0^k+ k\int_0^t X_s^{k-1} \Big(\eta - c_\mu X_s + \xi(X)_s\Big) ds
			+ \sum_{0<s\le t} \left\{X_s^k - X_{s-}^k \right\}
		\end{align*}
		where $X_{t}^k - X_{t-}^k =  \int_{\Rm_0} \left((X_{t-} + c_\nu X_{t-} z^2)^k - X_{t-}^k\right) N(dz, dt)
			= X_{t-}^k\int_{\Rm_0}  \Big((1+ c_\nu z^2)^k - 1 \Big) N(dz, dt).$
		Writing $E(t) := \Em\left[X_t^{k}\right]$, and 
		$K_k := k^{-1}\int_{\Rm_0} \Big((1+c_\nu z^2)^k -1 \Big) \Pi_L(dz)$, 
		we have
		\begin{align*}
		E(t)  
		&= E(0) 
			+k \Em\left[ \int_0^t X_s^{k-1}
			 \Big( \eta+ ( -  c_\mu+K_k) X_s \Big) ds\right]
			+ k\Em\left[ \int_0^t X_s^{k-1} \xi(X)_s ds 
				\right]=:\mathbf{I}+ \mathbf{II}.
			\numberthis\label{equation/1/proofs/1/stationarity/pqUI/E(t)}
		\end{align*}
		Let $C_k$ be given as in Lemma \ref{lemma/1/stationarity/cross} and suppose 
		\begin{align*}
			\lambda_k:= c_\mu - K_k 
				- \norm{f_\mu}_{L^1} - C_k \norm{f_\nu}_{L^k} >0.
		\end{align*}
		An exercise in calculus gives $\sup_{x\ge 0} kx^{k-1}\Big(\eta - \frac{1}{2}\lambda x\Big) = \eta^{k}\left(\frac{2 (k-1)}{k\lambda }\right)^{k-1} =:a_k$.
		% ,
		% and we write $a:= c+\epsilon$, for any $\epsilon>0.$
		Then for all $X_s\ge 0$,
		\begin{align*}
			k X_s^{k-1}\Big(
			\eta + \frac{1}{2}\left(-c_\mu + K_k
			+ \norm{f_\mu}_{L^1} +  C_k  \norm{f_\nu}_{L^k} \Big)
			 X_s \right) < a_k,
		\end{align*}
		from which we rearrange to get a bound for the integrand of $\mathbf{I}$:
		\begin{align*}
			&k X_s^{k-1}
			\Big(\eta+ ( - c_\mu+K_k) X_s \Big)
			< a_k - \frac{k}{2}\Big( c_\mu - K_k
			 + \norm{f_\mu}_{L^1} + C_k \norm{f_\nu}_{L^k} \Big) X_s^{k}.
			\numberthis\label{equation/1/proofs/1/stationarity/pqUI/bound_on_eta_term}
		\end{align*}
		For the integrand of $\mathbf{II}$,  Lemma \ref{lemma/1/stationarity/cross} gives the bound
		\begin{align*}
			&k\Em\left[X_s^{k-1} \xi(X)_s\right]
			\le 
			k\Big(\norm{f_\mu}_{L^1} + C_k \norm{f_\nu}_{L^k}\Big)\sup_{u\le s}\Em[X_u ^k].
		\end{align*}
		Combining this with \eqref{equation/1/proofs/1/stationarity/pqUI/E(t)} and \eqref{equation/1/proofs/1/stationarity/pqUI/bound_on_eta_term} 
		and writing $\bar E(s) = \sup_{u\le s} E(u)$,
		we have 
		\begin{align*}
			E(t)\le E(0)
			- \lambda_k'
			\int_0^t E(s) ds
			 +  \int_0^t\left( a_k+ \lambda_k''\bar E(s)\right) ds,
		\end{align*}
		where the constants $\lambda_k'$ and $\lambda_k''$ are given by
		\begin{align*}
			\lambda_k':  =  \frac{k}{2}\Big(c_\mu - K_k +  \norm{f_\mu}_{L^1} + C_k \norm{f_\nu}_{L^k} \Big),
			\quad
			\lambda_k'' :& =  k\Big(\norm{f_\mu}_{L^1} + C_k \norm{f_\nu}_{L^k}\Big).
		\end{align*}
		Our assumed condition \eqref{equation/1/moments/pqUIcondition} gives
		$\lambda_k' - \lambda_k''  = \frac{k}{2} \lambda_k >0$.
		By Lemma \ref{lemma/1/stationarity/ItoNisio} (\ref{lemma/1/stationarity/ItoNisio/1}), 
		\begin{align*}
			E(t)\le  E(0) + \int_0^t e^{-\lambda_k'(t-s)}  \left(a_k+\lambda_k''\bar E(s)\right) ds. 
			\numberthis\label{equation/1/proofs/1/stationarity/pqUI/E(t)afterfirstGronwall}
		\end{align*}
		Since $\bar E$ is non-decreasing and $\lambda_k'>0$, a quick integration by parts shows 
		\begin{align*}
			\int_0^t e^{-\lambda_k'(t-s)}  \left(a_k+\lambda_k''\bar E(s)\right) ds
			= \frac{(1-e^{-\lambda_k' t})(a_k + \lambda_k''\bar E(0))}{\lambda_1}
			+\frac{\lambda_k''}{\lambda_k'}\int_0^t \left(1-e^{-\lambda_k'(t-s)}\right)  d\bar E(s)
		\end{align*}
		is an non-decreasing function of $t$.
		Hence taking supremums in \eqref{equation/1/proofs/1/stationarity/pqUI/E(t)afterfirstGronwall}, we have
		\begin{align*}
			\bar E(t) = \sup_{u\in [0,t]} E(u) 
			& \le E(0) + \sup_{u\in [0,t]} \int_0^u e^{-\lambda_k'(u-s)}\left(a_k+\lambda_k''\bar E(s)\right) ds
			   \\
			% & \le E(0) + \int_0^t e^{-\lambda_1(t-s)} \left(a+\lambda_2\bar E(s)\right) ds
			   % \\
			& = \Em[X_0^k] + a_k \frac{1-e^{-\lambda_k' t}}{\lambda_k'}
			+ \lambda_k'' \int_0^t e^{-\lambda_k'(t-s)} \bar E(s)ds.
		\end{align*}
		By Lemma \ref{lemma/1/stationarity/ItoNisio} (\ref{lemma/1/stationarity/ItoNisio/2}), since $\lambda_k'>\lambda_k''>0$ and $\lambda_k' - \lambda_k'' = \frac{k}{2}\lambda_k$ for all $t\ge 0$, 
		\begin{align*}
			\bar E(t) \le \frac{2\lambda_k' }{k \lambda_k}\left(\Em[X_0^k] + a_k \frac{1-e^{-\lambda_k' t}}{\lambda_k'}\right) <\infty.
		\end{align*}

	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\pf{(\ref{theorem/1/moments/moment bound/L2}).}
	When $k=1$, we have $C_1 =\kappa_2$, $K_1 = c_\nu \int_{\Rm_0} z^2 \Pi_L(dz) = c_\nu\kappa_2$, $a_1 = 0$, so that
	% \begin{align*}
	% 	\lambda_1 = c_\mu - c_\nu \kappa_2 - \norm{f_\mu}_{L^1} - \kappa_2 \norm{f_\nu}_{L^1},
	% 	\quad \lambda_1'' = \norm{f_\mu}_{L^1} + \kappa_2 \norm{f_\nu}_{L^1},
	% \end{align*}
	% $\lambda_2 =  \norm{f_\mu}_{L^1} + \kappa_2 \norm{f_\nu}_{L^1}$,
	% $\lambda_1  =  \frac{1}{2}(c_\mu - c_\nu \kappa_2 +  \norm{f_\mu}_{L^1} + \kappa_2 \norm{f_\nu}_{L^1})$,
	% so that $\lambda_1 - \lambda_2 = \frac{1}{2}(c_\mu - c_\nu \kappa_2 -  \norm{f_\mu}_{L^1} - \kappa_2 \norm{f_\nu}_{L^1})$ 
	% and
	\begin{align*}
		\sup_{u\in[0,t]}\Em[X_u] 
		\le \frac{2 \lambda_k'}{k \lambda_k}\Em[X_0] 
		= \Em[X_0] 
		\left(
			1 +
			2\frac{\norm{f_\mu}_{L^1} + \kappa_2 \norm{f_\nu}_{L^1}}
			{c_\mu - c_\nu \kappa_2 -  \norm{f_\mu}_{L^1} - \kappa_2 \norm{f_\nu}_{L^1}}
		\right).
	\end{align*}
	Similarly, 
	when $k=2$, simple computations give $C_2 = \kappa_4$, 
	\begin{align*}
		&K_2  =  \int_{\Rm_0} \left(\frac{1}{2} c_{\nu}^2 z^4 + c_\nu z^2\right) \Pi_L(dz) 
			= \frac{1}{2}c_{\nu}^2\kappa_4 + c_\nu \kappa_2,
		\\
		&\lambda_2 = c_\mu - c_\nu \kappa_2 - \frac{1}{2}c_\nu^2 \kappa_4 - \norm{f_\mu}_{L^1} - \kappa_4 \norm{f_\nu}_{L^2},
	\end{align*}
	and $a_2 = \eta^2/\lambda_2$,
	% and
	% $\lambda_2  = 2(\norm{f_\mu}_{L^1} + \kappa_4 \norm{f_\nu}_{L^2})$
	% , 
	% $\lambda_1 = c_\mu - c_\nu \kappa_2 - \frac{1}{2}c_\nu^2 \kappa_4 - \norm{f_\mu}_{L^1} - \kappa_4 \norm{f_\nu}_{L^2}
	% $,
	so that
	\begin{align*}
		\sup_{u\in[0,t]}\Em[X_u^2] \le 
		\left(\frac{\eta}{\lambda_2}\right)^2
		+ \Em[X_0^2]\left(1+ \frac{2}{\lambda_2}\Big(\norm{f_\mu}_{L^1} + \kappa_4 \norm{f_\nu}_{L^2}\Big)\right).
	\end{align*}
	These bounds obviously do not depend on $t$. 
\end{proof}

==> proofs/proofs_strictstationarity.tex <==
%!TEX root = ../main.tex
	\subsection{Strict stationarity}
	We will write $\norm{\cdot}_\infty$ for the uniform norm on $\scD$ given by
	$\norm{f}_{\infty} := \sup_{u\in[-r,0]} |f(u)|$. Recall the segment process $_tX$ defined in Section \ref{section/1/stationarity}.
	\begin{proposition}\label{proposition/1/placeholder1}
		Suppose Theorem \ref{theorem/1/moments/moment bound}(\ref{theorem/1/moments/moment bound/L2uniform}) holds and $X$ is uniformly bounded in $L^2$. Then $\sup_{t\ge 0}\Em \norm{_tX}^2_\infty<\infty$.
	\end{proposition} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%	
\begin{proof}[Proof of Proposition \ref{proposition/1/placeholder1}]
	
\end{proof}



==> proofs/proofs_variance.tex <==
%!TEX root = ../main.tex
\subsection{Variance}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Applying It\^o's Lemma to $x\map x^2$, we have
	\begin{align*}
		dX(t)^2  & = 2X(t) \left(\eta -  c_0 X(t) + \int_{-p}^0 f(u)X_t(u)  du\right) dt 
		+ 2 c_\nu X(t-)^2 d\td S (t)
		+ c_\nu^2 X(t-) d[\td S,\td S](t),
	\end{align*}
	which gives
	\begin{align*}
		\Em\left[X(t)^2\right] & = \Em\left[X(0)^2\right] + 2 \eta \int_0^t \Em [X(s)] ds 
		+ (\kappa_4 c_\nu^2 - 2 c_0)\int_0^t \Em \left[X(s)^2\right] ds 
		   \\
		& \quad + 2\int_0^t \int_{-p}^0 f(u) \Em\left[X(s)X(s+u)\right] du ds.\numberthis\label{eq_p0/EX^2}
	\end{align*}
	Recall from \eqref{eq/pq_firstmoment/FDE}, the mean of the process $X$ satisfies
	\begin{align*}
		\dot m(t) = \eta - c_0 m(t) + \int_{-p}^0 f(u) m(s+u) du.
	\end{align*}
	Using the change of variable formula, 
	\begin{align*}
		m(t)^2 
		& =    m(0)^2 + 2\int_0^t m(s) \dot m(s) ds
		   \\
		& = m(0)^2 + 2 \eta\int_0^t m(s) ds - 2c_0 \int_0^t m(s)^2 ds 
+ 2\int_0^t\int_{-p}^0 f(u) m(s)m(s+u) du ds.\numberthis\label{eq_p0/mX^2}
	\end{align*}
	From here on, we will denote $V(t):= \Var(X(t))$ and $C(t):= \Cov(X(t), X(s))$. Combining \eqref{eq_p0/EX^2} and \eqref{eq_p0/mX^2}, we have
	\begin{align*}
		V(t)  & =   \Em(X(t)^2) - \Em(X(t))^2
		   \\
		& = 
		V(0) + (\kappa_4 c_\nu^2- 2c_0)\int_0^t V(s) ds + \kappa_4 c_\nu^2 \int_0^t m(s)^2 ds
		   \\
		& \quad + 2 \int_{0}^{t}\int_{-p}^0 f(u) C(s,s+u) du ds.\numberthis\label{eq_p0/V(t)}
	\end{align*}
	Differentiating, we have a functional differential equation for the variance
	\begin{align*}
		\frac{d}{dt} V(t) = \kappa_4 c_\nu^2  m^2  + (\kappa_4 c_\nu^2- 2c_0)V(t) 
		+ 2 \int_{-p}^0 f(u) C(t,t+u) du,\numberthis\label{eq_p0/dV(t)}
	\end{align*}
	with initial condition $\{C(0, u), u\in [-p,0]\}$. 
	
	\subsubsection{Covariance of CDGARCH(p,0)}
	For $t>0$ and some fixed $h>0$, we can write
	\begin{align*}
		\Em[X(t)X(t+h)] & =  \Em[X(t)^2] + \Em[X(t) (X(t+h) - X(t))].
	\end{align*}
	From \eqref{eq/pq_stationarity/p0X}, the second term can be written as 
	\begin{align*}
		X(t) (X(t+h) - X(t))& =\int_{t}^{t+h}X(t) dX(s)   
			\\
		& = \int_t^{t+h} X(t)  \left( \eta - c_0 X(s) + \int_{-p}^0 f(u)X(s+u) du \right) ds
		   \\
		& \quad + c_\nu \int_t^{t+h} \int_{\Rm_0}  X(t)X(s-) z^2 \td N(dz,ds).
	\end{align*}
	Therefore,
	\begin{align*}
		\Em[X(t)X(t+h)] & =  \Em[X(t)^2] + \eta h \Em[X(t)] - c_0 \int_{t}^{t+h} \Em[X(t)X(s)] ds
		   \\
		& \quad + \int_{t}^{t+h} \int_{-p}^0 f(u) \Em[X(t) X(s+u)] du ds. \numberthis\label{eq_p0/EX(t)EX(t+h)}
	\end{align*}
	Similarly, 
	\begin{align*}
		m(t)m(t+h)  & =m(t)^2 + m(t)\left(m(t+h) - m(t)\right)
		   \\
		& =  m(t)^2 + \int_{t}^{t+h} m(t) dm(s)
		   \\
		& =   m(t)^2 + \eta h m(t) - c_0 \int_t^{t+h} m(t) m(s) ds 
		   \\
		& \quad +
		\int_t^{t+h} \int_{-p}^0 f(u) m(t)m(s+u)du ds.\numberthis\label{eq_p0/m(t)m(t+h)}
	\end{align*}
	Putting \eqref{eq_p0/EX(t)EX(t+h)} and \eqref{eq_p0/m(t)m(t+h)} together, we have
	\begin{align*}
		C(t,t+h) & =  V(t) -c_0 \int_t^{t+h} C(t,s) ds + \int_t^{t+h} \int_{-p}^0 f(u)C(t, s+u) du ds
		   \\
		& = V(t) -c_0 \int_0^{h} C(t,t+s) ds + \int_0^{h} \int_{-p}^0 f(u)C(t, t+s+u) du ds. 
		\numberthis\label{eq_p0/C(t,t+h)}
	\end{align*}
	Differentiating, we have
	\begin{align*}
		\frac{d}{dh} C(t,t+h) =-c_0 C(t,t+h) + \int_{-p}^0 f(u) C(t,t+h+u) du,
	\end{align*}
	and
	\begin{align*}
		\frac{d}{dt} C(t,t+h) =\frac{d}{dt}V(t) -c_0\int_0^h \frac{d}{dt} C(t,t+s)  ds
		 + \int_0^h\int_{-p}^0 f(u)\frac{d}{dt} C(t,t+s+u) du ds,
	\end{align*}
	\subsubsection{Stationary regime of CDGARCH(p,0)}
	Assuming $X$ is second order stationary, i.e. 
	\begin{align*}
		V(t)=V, \quad m(t) = m = \frac{\eta}{c_0 - \int_{-p}^0f(u)du},\qand C(t,s) = C(t-s),
	\end{align*}
	the equation \eqref{eq_p0/dV(t)} becomes
	\begin{align*}
		V  = \frac{1}{(2c_0-\kappa_4c_\nu^2)} 
		\left(\frac{\kappa_4 c_\nu^2 \eta^2}{\left(c_0 - \int f(u)du\right)^2} + 2\int_{-p}^0 f(u) C(u) du\right),
	\end{align*}
	or as a equation of the covariance,
	\begin{align*}
		\int_{-p}^0  C(u)f(u) du& = 
		\left(c_0-\frac{\kappa_4c_\nu^2}{2}\right)V -\frac{\kappa_4 c_\nu^2 \eta^2}{2\left(c_0 - \int f(u)du\right)^2},
	\end{align*}
	i.e., if we let $k_0= - (c_0 - \kappa_4 c_\nu^2/2)$ and 
	$k_1 = -\frac{\kappa_4 c_\nu^2 \eta^2}{2\left(c_0 - \int f(u)du\right)^2}$, we have
	\begin{align*}
		k_0 C(0) + \int_{-p}^0 f(u) C(u) du = k_1
	\end{align*}
	For the covariance, \eqref{eq_p0/C(t,t+h)} becomes
	\begin{align*}
		C(h) & =  V - c_0 \int_t^{t+h} C(s-t) ds + \int_t^{t+h} \int_{-p}^0f(u) C(s+u-t) du ds
		   \\
		& = C(0) - c_0 \int_0^{h} C(s) ds + \int_0^{h} \int_{-p}^0f(u) C(s+u) du ds.
	\end{align*}
	The process $X$ is mean square continuous so the covariance function $C$ is continuous.  Therefore, the stationary covariance satisfies the functional differential equation
	\begin{align*}
		\frac{d}{dh} C(h)  = -c_0 C(h) + \int_{-p}^0 f(u)C(h+u) du,
	\end{align*}
	with initial condition $\{C(u), u\in [-p,0]\}$ that satisfies
	\begin{align*}
		k_0 C(0) + \int_{-p}^0 f(u) C(u) du = k_1
	\end{align*}
	\begin{align*}
		\Delta(z) = z -\int_{[-r,0]} e^{zu} (\mu+ \kappa_2 \nu)(du)
	\end{align*}
	stable if $c_0 > \norm{f}_{L^1}$
	so this converges to zero exponentially fast


	

==> results/1.tex <==
%!TEX root = ../main.tex
\subsection{Strict stationarity}\label{section/1/stationarity}
We first introduce some notations and concepts. Recall the definitions for $c_\mu, c_\nu, f_\mu$ and $f_\nu$ in \eqref{equation/1/model/mu} and \eqref{equation/1/model/nu}. From here on, we will write $c_0:= c_\mu - \kappa_2 c_\nu$ and $f:= f_\mu+ \kappa_2 f_\nu$. Since $f_\mu$ and $f_\nu$ are supported on $[-p,0]$ and $[-q,0]$ respectively, writing $r=p\maxx q$, 
	\begin{align*}
		(\mu+ \kappa_2 \nu)(E)=-c_0 \delta_0(E) + \int_{E\cap [-r,0]} f(u)du
		,\quad\forall E\in \cB([-r,0]).
	\end{align*}
Recalling $S_t = \td S_t + \kappa_2 t$, we rewrite the process $\xi(X)$ defined in \eqref{equation/1/semimartingale/xi} as
\begin{align*}
	\xi(X)_t = \int_{t-r}^t f(u-t) X_u du + \int_{t-q+}^t f_\nu(u-t) X_{u-} d\td S_u,\quad t\ge 0, 
\end{align*}
and the SDDE \eqref{equation/1/semimartingale/XSDDE} for the variance process as
\begin{align*}
	dX_t = \Big(\eta - c_0 X_t + \xi(X)_t\Big) dt + c_\nu X_{t-} d\td S_t, \quad t\ge 0,
	\numberthis\label{equation/1/stationarity/X}
\end{align*}
with initial condition $X = \Phi$ on $[-r,0]$.

We endow $\scD=\scD_{[-r,0]}$ with the Skorokhod metric $d^\circ$ (see \citet{Billingsley2013}), under which $\scD$ is Polish, i.e. separable and complete.
Let $\cP(\scD)$ be the (Polish) space of finite Borel measures on $\scD$ and $\scB_b(\scD)$ (resp. $\scC_b(\scD)$) be the class of bounded Borel measurable (resp. bounded continuous) functions on $(\scD,d^\circ)$. 
Write $\<\cdot, \cdot\>$ for duality pairing 
$\< P, g\> := \int_\scD g(\phi) dP(\phi)$ for $g\in \scB_b(\scD)$ and $P\in\cP(\scD)\subset\scB_b(\scD)^*$. Let $\mathrm{Lip}(\scD)$ (resp. $\Lip_b(\scD)$) be the space of real valued Lipschitz (resp. bounded Lipschitz) functions on $\scD$.

From the expression \eqref{equation/1/semimartingale/XSDDE}, it is easy to see that the process $(X_t)_{t\ge 0}$ is not a Markov process so the usual practice is to ``lift'' $X$ up into a functional space so that it has the Markov property. 
Define the $\scD$-valued \textit{segment process} $(_tX)_{t\ge 0}$ 
by $_tX_u^\Phi=X_{t+u}^\Phi, u\in[-r,0]$, where $X_{\bigcdot}^\Phi$ is the solution to \eqref{equation/1/semimartingale/XSDDE} with initial condition $\Phi$.
It is straightforward to show that $(_tX)_t$ is a Markov process on $\scD$ (see for instance Prop. 3.3 of \cite{ReissRiedlevanGaans2006}). 

Write $(P_t)_{t\ge 0}$ for the Markovian semigroup on $\scB_b(\scD)$ generated by $(_tX)_{t\ge 0}$, i.e., $P_t g(\phi) := \Em\left[g(_tX^\phi)\right]$ for any $g\in \scB_b(\scD)$ and $\phi\in\scD$. If $\pi$ is the distribution of initial condition $\Phi$, then the distribution of $_tX^\Phi$ is given by $P^*_t\pi$, where $P^*_t$ is the adjoint semigroup on $\cP(\scD)$ defined by
$\< P^*_t\mu, g\> = \left< \mu, P_t g \right>$, for any $g\in \scB_b(\scD)$. 
Finally, a \textit{stationary} or \textit{invariant distribution} $\pi$ of $(_tX)_t$ is a probability measure $\pi\in\cP(\scD)$ such that $P_t^* \pi = \pi$, that is, $\left< \pi, g\right> = \left<\pi, P_t g\right>$ for any $g\in \scB_b(\scD)$. 

\begin{remark}
	There exists extensive literature on the existence, uniqueness, and ergodicity of stationary distributions to Markov processes in Polish spaces (see for instance \citet{DaPratoZabczyk1996}). A conventional way to establish existence of an invariant measure is through the so-called Feller property of the Markovian semigroup, while the strong Feller property ensures uniqueness. Difficulties arise for SFDEs like \eqref{equation/1/stationarity/X} driven by discontinuous noise. Here, the Markov semigroup is typically only eventually Feller, and not eventually strongly Feller (see \cite{ReissRiedlevanGaans2006}). The classical results are not readily applicable to the CDGARCH equations, instead, we utilize a relatively new result by \citet*{BaoYinYuanEtAl2014}.
	\qed
\end{remark}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}\label{theorem/1/stationarity} 
	Suppose $\kappa_4<\infty$ and \eqref{equation/1/moments/pqUIcondition} holds for $k=2$, i.e.,
	\begin{align*}
	 	c_0> \norm{f}_{1}
		+ \kappa_4\norm{f_\nu}_{2}+ \frac{\kappa_4c_\nu^2}{2}   \numberthis\label{condition/1/stationarity/strictstationary}
	\end{align*} 
	so that $X$ uniformly bounded in $L^2$ by Theorem \ref{theorem/1/moments/moment bound} (\ref{theorem/1/moments/moment bound/Lk pq}). Then we have
	\begin{enumerate}[(i)]
	 	\item \label{theorem/1/stationarity/stationarity}  The process $(_tX)_{t\ge 0}$ admits a unique stationary distribution $\pi$ on $\scD$, i.e., $\exists ! \pi\in\cP(\scD)$ with
	 		\begin{align*}
	 			\int_{\scD} F(_t X^\phi) \pi(d \phi) = \int_{\scD} F(\phi) \pi(d \phi), \quad \forall F\in\scB_b(\scD). 
	 		\end{align*}
	 	\item \label{theorem/1/stationarity/exponential ergodicity}  Furthermore, $\pi$ is exponentially ergodic, i.e. for any initial condition $\phi\in\scD$, there exist constant $C_\phi$ and $\lambda>0$ such that for all $t>r$, 
		\begin{align*}
			\left|P_t F(\phi) - \< \pi, F\> \right|
			\le C_\phi e^{-\lambda t}\norm{F}_{\mathrm {Lip}},\quad \forall F\in\mathrm{Lip}(\scD).\qed
		\end{align*}
	 \end{enumerate}
\end{theorem} 

\begin{remark}
	Let $\pi\in\cP(\scD)$ be a stationary distribution of $(_tX)_{t\ge 0}$ on $\scD$, from $\pi$, we can always construct a stationary distribution of the real valued processes $(X_t)_{t\ge 0}$. 
	Let $E_0: \scD\to\Rm$ be the point evaluation map  $\phi\mapsto \phi(0)$, then for any $F\in \scB_b(\Rm)$, the composition $F\circ E_0$ is in $\scB_b(\scD)$.
	Let $\pi_0$ be the image measure on $\Rm$ of $\pi$ under $E_0$, i.e., $\pi_0([a,b]) = \pi(\{\phi\in \scD : \pi(0)\in[a,b]\})$, for any $[a,b]\subseteq \Rm$. 
	Suppose the $\scD$-valued initial value $\Phi$ has distribution $\cL(\Phi) = \pi$, then it is clear that the real valued random variable $\Phi_0$ has distribution $\cL(\Phi_0) = \pi_0$ and 
	\begin{align*}
		\Em\left[F\left(X_t^\Phi\right)\right]    
		& =   \Em\left[(F\circ E_0)\left(_tX^\Phi\right)\right] 
		= \left<\pi, P_t(F\circ E_0) \right>, \quad F\in \scB_b(\Rm). 
	\end{align*} 
	Hence for any $F\in\scB_b(\Rm)$, by the stationarity of $\pi$, 
	\begin{align*}
		\Em\left[F(X_t^\Phi )\right]    
		& = \left<\pi, P_t(F\circ E_0) \right>
		= \left<\pi, F\circ E_0\right>  = \Em\left[F(X_0^\Phi)\right], 
	\end{align*} 
	and we see that $\pi_0$ is a stationary distribution of $(X_t)_{t\ge 0}$. \qed
\end{remark}
	

	\begin{remark}
		From Theorem \ref{theorem/1/stationarity}, 
		if $X$ is covariance stationary, then it is automatically strict stationary as well, since it would be uniformly bounded in $L^2$. 
		On the other hand, it is clear that the condition \eqref{condition/1/stationarity/strictstationary} implies that the process $X$ is covariance stationary as well. Hence if we want the process $X$ to be highly persistent and not covariance stationary, then necessarily $\sup_t \Em[X_t^2]=\infty$. \qed
	\end{remark}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55






















==> results/results_stationarity.tex <==
%!TEX root = ../main.tex
\subsection{Strict stationarity}\label{section/1/stationarity}
% We first introduce some notations and concepts. Recall the definitions for $c_\mu, c_\nu, f_\mu$ and $f_\nu$ in \eqref{equation/1/model/mu} and \eqref{equation/1/model/nu}. From here on, we will write $c_0:= c_\mu - \kappa_2 c_\nu$ and $f:= f_\mu+ \kappa_2 f_\nu$. Since $f_\mu$ and $f_\nu$ are supported on $[-p,0]$ and $[-q,0]$ respectively, writing $r=p\maxx q$, 
% 	\begin{align*}
% 		(\mu+ \kappa_2 \nu)(E)=-c_0 \delta_0(E) + \int_{E\cap [-r,0]} f(u)du
% 		,\quad\forall E\in \cB([-r,0]).
% 	\end{align*}
% Recalling $S_t = \td S_t + \kappa_2 t$, we rewrite the process $\xi(X)$ defined in \eqref{equation/1/semimartingale/xi} as
% \begin{align*}
% 	\xi(X)_t = \int_{t-r}^t f(u-t) X_u du + \int_{t-q+}^t f_\nu(u-t) X_{u-} d\td S_u,\quad t\ge 0, 
% \end{align*}
% and the SDDE \eqref{equation/1/semimartingale/XSDDE} for the variance process as
% \begin{align*}
% 	dX_t = \Big(\eta - c_0 X_t + \xi(X)_t\Big) dt + c_\nu X_{t-} d\td S_t, \quad t\ge 0,
% 	\numberthis\label{equation/1/stationarity/X}
% \end{align*}
% with initial condition $X = \Phi$ on $[-r,0]$.
We first introduce some notations.
We endow $\scD=\scD_{[-r,0]}$ with the Skorokhod metric $d^\circ$ (see \citet{Billingsley2013}), under which $\scD$ is Polish, i.e. separable and complete.
Let $\cP(\scD)$ be the (Polish) space of finite Borel measures on $\scD$ and $\scB_b(\scD)$ (resp. $\scC_b(\scD)$) be the class of bounded Borel measurable (resp. bounded continuous) functions on $(\scD,d^\circ)$. 
Write $\<\cdot, \cdot\>$ for duality pairing 
$\< P, g\> := \int_\scD g(\phi) dP(\phi)$ for $g\in \scB_b(\scD)$ and $P\in\cP(\scD)\subset\scB_b(\scD)^*$. Let $\mathrm{Lip}(\scD)$ (resp. $\Lip_b(\scD)$) be the space of real valued Lipschitz (resp. bounded Lipschitz) functions on $\scD$.


Let $(P_t)_{t\ge 0}$ be the Markovian semigroup on $\scB_b(\scD)$ generated by $(X_{(t)})_{t\ge 0}$, i.e., $P_t g(\phi) := \Em[g(X_{(t)}^\phi)]$ for any $g\in \scB_b(\scD)$ and $\phi\in\scD$. If $\pi$ is the distribution of initial condition $\Phi$, then the distribution of $X_{(t)}^\Phi$ is given by $P^*_t\pi$, where $P^*_t$ is the adjoint semigroup on $\cP(\scD)$ defined by
$\< P^*_t\mu, g\> = \left< \mu, P_t g \right>$, for any $g\in \scB_b(\scD)$ and $\mu\in \cP(\scD)$. 
Finally, a \textit{stationary} or \textit{invariant distribution} $\pi$ of $(X_{(t)})_t$ is a probability measure $\pi\in\cP(\scD)$ such that $P_t^* \pi = \pi$, that is, $\left< \pi, g\right> = \left<\pi, P_t g\right>$ for any $g\in \scB_b(\scD)$. 

\begin{remark}
	There exists extensive literature on the existence, uniqueness, and ergodicity of stationary distributions of Markov processes in Polish spaces (see for instance \citet{DaPratoZabczyk1996}). A conventional way to establish existence of an invariant measure is through the so-called Feller property of the Markovian semigroup, while the strong Feller property ensures uniqueness. Difficulties arise for SFDEs like \eqref{equation/1/semimartingale/XSDDE} driven by discontinuous noise. Here, the Markov semigroup is typically only eventually Feller, and not eventually strongly Feller (see \cite{ReissRiedlevanGaans2006}). The classical results are not readily applicable to the CDGARCH equations.
	\qed
\end{remark}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}\label{theorem/1/stationarity} 
	Suppose $\kappa_4<\infty$ and condition \eqref{condition/1/moments/L1uniform} holds
	so that $\sup_{t\ge 0}\Em \norm{X_{(t)}}_{\infty}^2<\infty$ by Theorem \ref{theorem/1/moments/moment bound}(\ref{theorem/1/moments/moment bound/segment process}). 
	Then the following holds.
	\begin{enumerate}[(a)]
	 	\item \label{theorem/1/stationarity/stationarity}  The process $(X_{(t)})_{t\ge 0}$ admits a unique stationary distribution $\pi$ on $\scD$, i.e., $\exists ! \pi\in\cP(\scD)$ with
	 		\begin{align*}
	 			\int_{\scD} F(X_{(t)}^\phi) \pi(d \phi) = \int_{\scD} F(\phi) \pi(d \phi), \quad \forall F\in\scB_b(\scD). 
	 		\end{align*}
	 	\item \label{theorem/1/stationarity/exponential ergodicity}  Furthermore, $\pi$ is exponentially ergodic, i.e. for any initial condition $\phi\in\scD$, there exist constant $C_\phi$ and $\lambda>0$ such that for all $t>r$, 
		\begin{align*}
			\left|P_t F(\phi) - \< \pi, F\> \right|
			\le C_\phi e^{-\lambda t}\norm{F}_{\mathrm {Lip}},\quad \forall F\in\mathrm{Lip}(\scD).\qed
		\end{align*}
	 \end{enumerate}
\end{theorem} 

\begin{remark}
	Let $\pi\in\cP(\scD)$ be a stationary distribution of $(X_{(t)})_{t\ge 0}$ on $\scD$. From $\pi$, we can always construct a stationary distribution of the real valued processes $(X_t)_{t\ge 0}$. 
	Let $E_0: \scD\to\Rm$ be the point evaluation map  $\phi\mapsto \phi(0)$, then for any $F\in \scB_b(\Rm)$, the composition $F\circ E_0$ is clearly in $\scB_b(\scD)$.
	Let $\pi_0$ be the image measure on $\Rm$ of $\pi$ under $E_0$, i.e., $\pi_0([a,b]) = \pi(\{\phi\in \scD : \pi(0)\in[a,b]\})$, for any $[a,b]\subseteq \Rm$. 
	Suppose the $\scD$-valued initial value $\Phi$ has distribution $\cL(\Phi) = \pi$, then it is clear that the real valued random variable $\Phi_0$ has distribution $\cL(\Phi_0) = \pi_0$ and 
	\begin{align*}
		\Em\left[F\left(X_t^\Phi\right)\right]    
		& =   \Em\left[(F\circ E_0)\left(X_{(t)}^\Phi\right)\right] 
		= \left<\pi, P_t(F\circ E_0) \right>, \quad F\in \scB_b(\Rm). 
	\end{align*} 
	Hence for any $F\in\scB_b(\Rm)$, by the stationarity of $\pi$, 
	\begin{align*}
		\Em\left[F(X_t^\Phi )\right]    
		& = \left<\pi, P_t(F\circ E_0) \right>
		= \left<\pi, F\circ E_0\right>  = \Em\left[F(X_0^\Phi)\right], 
	\end{align*} 
	and we see that $\pi_0$ is a stationary distribution of $(X_t)_{t\ge 0}$. \qed
\end{remark}
	

	\begin{remark}
		If $X$ is covariance stationary, then obviously it is uniformly bounded in $L^2$ and hence strictly stationary by Theorem \ref{theorem/1/moments/moment bound} and Theorem \ref{theorem/1/stationarity}. 
		\qed
	\end{remark}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55






















==> results/results_variance.tex <==
%!TEX root = ../main.tex
\subsection{Second order behavior of X}\label{section_proofs/variance}
